Rethinking Personalized Reward Modeling for LLMs under Preference Heterogeneity via Group-Debiased Federated Learning

Large language models are increasingly aligned to human preferences via reward modeling, but user preference data are sensitive and often cannot be centralized. Federated learning keeps such data local while learning a shared initial reward model, which is later personalized for each client through local fine-tuning. Because users often assign opposite labels to the same pair of responses, existing federated methods address preference heterogeneity by clustering similar clients and training one reward model per group, assuming that each group requires its own initialization. We show that this assumption is unnecessary. Under balanced preference groups, a single FedAvg model, despite starting at nearly random accuracy, surpasses reward models trained separately for each ground-truth group after only a few local optimization steps. We attribute this phenomenon to the flatness of the shared initialization: averaging across all clients learns richer shared representations that distinguish responses while canceling conflicting preference directions, leaving the model near a decision boundary that can be rapidly adapted. Group imbalance breaks this effect as the cancellation becomes asymmetric and leaves minority clients too far from the boundary to recover. Motivated by this observation, we propose FedGD (Federated Learning with Group Debiasing), which discovers latent preference groups during federated training and learns a single reward model using group-debiased client sampling. By counteracting the effect of group imbalance, FedGD learns an initialization that remains highly adaptable, enabling effective personalization without prior knowledge of the underlying groups.

==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/command/math_command.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


% Customized Math
\DeclareMathOperator{\Tr}{Tr}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\let\ab\allowbreak

\newcommand{\trace}{\Tr}


==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/command/mycommand.tex <==
\newcommand{\mytitle}{Rethinking Personalized Reward Modeling for LLMs under Preference
Heterogeneity via Group-Debiased Federated Learning}

\newcommand{\myabbtitle}{\mytitle}
\newcommand{\alg}{\textbf{\code{FedGD}}\xspace}
\newcommand{\algft}{\textbf{\code{FedGD-FT}}\xspace}

\newcommand{\acc}[2]{#1_{\pm #2}}   % \acc{84.10}{5.43} → 84.10_{±5.43}


\newcommand{\solidline}{--}
\newcommand{\dotline}{{\tiny \makebox[3mm]{$\cdots$}}}

\makeatletter
\renewcommand\@fnsymbol[1]{%
  \ifcase#1\or $\dagger$\or $\ddagger$\or $\S$\or $\P$\or $\|$\or
  $\ast\ast$\or $\dagger\dagger$\or $\ddagger\ddagger$\else\@ctrerr\fi}
\makeatother


\setlength{\textfloatsep}{10pt plus 2pt minus 2pt}
\setlength{\dbltextfloatsep}{10pt plus 2pt minus 2pt}
\setlength{\floatsep}{8pt plus 2pt minus 2pt}
\setlength{\intextsep}{8pt plus 2pt minus 2pt}


% \usepackage{geometry}
% \usepackage{subfig}
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{bbm}
\usepackage{mathtools}
% \usepackage{amsthm}
\usepackage{nccmath}
\usepackage{setspace}
\usepackage[T1]{fontenc}
\usepackage[scaled]{beramono}
% \usepackage{caption}
\usepackage{subcaption}

\usepackage[ruled,linesnumbered]{algorithm2e} % 


% \usepackage{tikz}
% \definecolor{petalcolor}{HTML}{F5F0E6}
% \definecolor{petaledge}{HTML}{2B2B2B}
% \definecolor{corecolor}{HTML}{F2B705}
% \definecolor{coredeep}{HTML}{C98A00}
% \definecolor{corelight}{HTML}{FFD95C}

% \newcommand{\daisyspin}{135}    % 빈 자리 각도 (7시 반)
% \newcommand{\daisysize}{1.45}   % 전체 크기 배율

% \newcommand{\daisy}{%
%   \begin{tikzpicture}[baseline=-0.38ex,
%                       x=\daisysize ex, y=\daisysize ex,
%                       rotate=\daisyspin]
%     \foreach \a in {36,72,...,324}{%
%       \fill[petalcolor, draw=petaledge, line width={\daisysize*0.06ex}, rotate=\a]
%         (0,0.78) ellipse [x radius=0.29, y radius=0.56];}%
%     \fill[corecolor, draw=petaledge, line width={\daisysize*0.06ex}] (0,0) circle (0.40);%
%     \fill[corelight] (0,0) circle (0.26);%
%     \foreach \a in {0,45,...,315}{\fill[coredeep] (\a:0.155) circle (0.033);}%
%     \foreach \a in {22.5,67.5,...,337.5}{\fill[coredeep] (\a:0.30) circle (0.030);}%
%   \end{tikzpicture}%
% }

\usepackage{tikz}
\definecolor{petalcolor}{HTML}{F5F0E6}
\definecolor{petaledge}{HTML}{2B2B2B}
\definecolor{corecolor}{HTML}{F2B705}
\definecolor{coredeep}{HTML}{C98A00}
\definecolor{corelight}{HTML}{FFD95C}

\newcommand{\daisyspin}{135}
\newcommand{\daisysize}{1.45}

\newcommand{\daisy}{%
  \begin{tikzpicture}[baseline=-0.48ex,
                      x=\daisysize ex, y=\daisysize ex,
                      rotate=\daisyspin]
    \foreach \a in {36,72,...,324}{%
      \fill[petalcolor, draw=petaledge, line width={\daisysize*0.06ex}, rotate=\a]
        (0,0.78) ellipse [x radius=0.29, y radius=0.56];}%
    \fill[corecolor, draw=petaledge, line width={\daisysize*0.06ex}] (0,0) circle (0.40);%
    \fill[corelight] (0,0) circle (0.26);%
    \foreach \a in {0,45,...,315}{\fill[coredeep] (\a:0.155) circle (0.033);}%
    \foreach \a in {22.5,67.5,...,337.5}{\fill[coredeep] (\a:0.30) circle (0.030);}%
  \end{tikzpicture}%
}





\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\newcommand{\algcapsty}[1]{\small\sffamily\bfseries{#1}}
\SetAlCapSty{algcapsty}

\usepackage[T1]{fontenc}
\usepackage{wrapfig,lipsum,booktabs}

% \usepackage{natbib}
\usepackage{soul}
\usepackage{dsfont}
\usepackage{enumitem}

% \usepackage{kotex}
% \usepackage{hyperref}
% \usepackage[hidelinks]{hyperref}
\usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amsfonts}
% \usepackage{arabtex}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage[Symbol]{upgreek}
\usepackage{lscape}
\usepackage{caption}
\usepackage{balance}
\usepackage{xspace}
\usepackage{float}


\usepackage{lipsum}



\usepackage{wasysym}
% \usepackage[table,xcdraw,dvipsnames]{xcolor}
\usepackage{multirow}
\usepackage{array, boldline, rotating}
\usepackage[table]{xcolor}   % \rowcolor 사용
\definecolor{flhl}{RGB}{219,234,254}  % 옅은 파랑 (원하는 색으로 조정)
\definecolor{fthl}{RGB}{253,230,203}   % 연주황



\let\Bbbk\relax % avoid clash with newtxmath (loaded by acmart) redefining \Bbbk
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\textcolor{green}{\ding{51}}\xspace}%
\newcommand{\xmark}{\textcolor{red}{\ding{55}}\xspace}%

\newcommand{\ds}[1]{\mathds{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbbm{#1}}




% %%%%%% Theorem Related Things %%%%%%
% \theoremstyle{plain}
% \newtheorem{thm}{Theorem}
% \newtheorem{cor}{Corollary}
% \newtheorem{lem}{Lemma}
% \newtheorem{prop}{Proposition}

% \theoremstyle{definition}
% \newtheorem{defn}{Definition}
% \newtheorem{assum}{Assumption}



\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Blue}{rgb}{0, 0.5, 1}
\definecolor{Green}{rgb}{0.0, 0.8, 0.0 }
\definecolor{Red}{rgb}{0.95, 0.55, 0.6}
\definecolor{Skyblue}{rgb}{0.6, 0.6, 0.95 }


% Citation

% \let\oldeqcite\cite
% \renewcommand*\cite[1]{(\oldcite{#1})}
\let\oldeqref\eqref
\renewcommand*\eqref[1]{(\ref{#1})}

% % Highlight (incl. note)
\newcommand{\ahn}[1]{\textcolor{ForestGreen}{$\rightarrow$SM:#1}}
\newcommand{\minchan}[1]{\textcolor{RoyalPurple}{$\rightarrow$MC:#1}}
\newcommand{\sungnyun}[1]{{\color{RoyalBlue}$\rightarrow$SK: #1}}
\newcommand{\eg}{\emph{e.g.,~}}
\newcommand{\ie}{\emph{i.e.,~}}


% % Separation (paragraph)
\newcommand{\myparagraph}[1]{\vspace{0.07cm}\noindent\textbf{#1}~}

% % math op.

% % Font
\def\code#1{\texttt{#1}}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

% % % Definition
% \theoremstyle{definition}




\newcommand{\thickhline}{\hlineB{4}}
\newcommand{\bfcode}[1]{\code{\textbf{#1}}}


% \definecolor{LightCyan}{rgb}{0.88,1,1}


% Supplementary title
\NewDocumentCommand{\supptitle}{s}{
\onecolumn
\begin{center}
    % \rule{\textwidth}{0.07cm}\\[-0.34cm]
    \rule{\textwidth}{0.03cm}\\[0.1cm]
    - Appendix -\\[0.2cm]
    {\Large 
        \textbf{\mytitle }
    }\\%[0.40cm]
    \rule{\textwidth}{0.03cm}\\[0.2cm]
\end{center}
}


==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/00_abstract.tex <==
\begin{abstract}
% Large language models are increasingly aligned to human preferences via reward
% modeling, but preference data are sensitive and often cannot be centralized.
% Federated learning keeps such data local, and personalization is obtained by
% fine-tuning a shared model on each client. Users often assign opposite labels to the
% same pair of responses, and existing federated methods handle such preference
% heterogeneity by clustering similar clients and training one model per group, so that
% no model has to average over conflicting labels. We show that group-specific
% initialization is not what makes a good initialization. Under balanced preference
% groups, a single FedAvg model starts at the level of random guessing yet surpasses a
% centralized model trained per ground-truth group within a few local steps. The reason
% is flatness: clients agree on what distinguishes the two responses and disagree only
% on which one is preferable, so averaging preserves the shared distinction, cancels the
% conflicting judgments, and leaves the model near the decision boundary. Group
% imbalance destroys this flatness, as the cancellation becomes asymmetric and leaves
% minority clients too far from the boundary to recover. We therefore propose \alg\
% (\textbf{Fed}erated Learning with \textbf{G}roup \textbf{D}ebiasing), which discovers
% the preference groups during federated training and trains a single reward model
% under group-debiased sampling over the discovered partition, restoring flatness
% without prior knowledge of the groups.


Large language models are increasingly aligned to human preferences via reward modeling, but user preference data are sensitive and often cannot be centralized.
Federated learning keeps such data local while learning a shared initial reward model, which is later personalized for each client through local fine-tuning.
Because users often assign opposite labels to the same pair of responses, existing federated methods address preference heterogeneity by clustering similar clients and training one reward model per group, assuming that each group requires its own initialization. 
We show that this assumption is unnecessary. 
Under balanced preference groups, a single FedAvg model, despite starting at nearly random accuracy, surpasses reward models trained separately for each ground-truth group after only a few local optimization steps. 
We attribute this phenomenon to the flatness of the shared initialization: averaging across all clients learns richer shared representations that distinguish responses while canceling conflicting preference directions, leaving the model near a decision boundary that can be rapidly adapted.
Group imbalance breaks this effect as the cancellation becomes asymmetric and leaves minority clients too far from the boundary to recover. 
Motivated by this observation, we propose \alg\ (\textbf{Fed}erated Learning with \textbf{G}roup \textbf{D}ebiasing), which discovers latent preference groups during federated training and learns a single reward model using group-debiased client sampling. By counteracting the effect of group imbalance, \alg\ learns an initialization that remains highly adaptable, enabling effective personalization without prior knowledge of the underlying groups.






\end{abstract}

==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/01_introduction.tex <==
\section{Introduction}

%  LLM alignment → reward model → data sensitivity → FL
Large language models (LLMs) are increasingly deployed in human-facing systems, where alignment with human preferences is crucial to user safety and satisfaction~\citep{bai2022constitutional,askell2021general,casper2023open}. A standard alignment pipeline typically trains a \emph{reward model} to predict human preferences and then optimizes the LLM through RLHF methods~\citep{schulman2017proximal,ouyang2022training}. However, preference data are highly sensitive and often cannot be centralized due to data-protection regulations~\citep{regulation2016regulation, illman2019california} and cross-jurisdictional sharing constraints~\citep{kopf2023openassistant}. Federated learning (FL)~\citep{mcmahan2017communication,li2020fedprox,kairouz2021advances}
offers a practical alternative: data remain local while a coordinating server aggregates model updates from decentralized clients.

% FL-based LLM alignment → single LLM limitation → need for personalized reward models
Existing FL-based preference alignment methods~\citep{fan2024fedrlhf,wu2024towards} struggle with \emph{preference heterogeneity} because they ultimately produce a single global LLM. For instance, FedRLHF~\citep{fan2024fedrlhf} shows clear performance degradation under severe heterogeneity. Even FedBiscuit~\citep{wu2024towards}, which uses multiple server-side reward models to label unlabeled response pairs, aggregates these signals into a single consensus to train one LLM via DPO~\citep{rafailov2023direct}. Consequently, existing methods fail to represent individual user preferences, underscoring the need for \emph{personalized reward models} tailored to each client.


% personalized FL → distinction under preference heterogeneity → research question
Recent personalized FL (PFL) methods~\citep{oh2021fedbabu,dong2022spherefed,kim2023fedfn,kim2025feddr} widely adopt a two-stage strategy: pre-training a single shared model globally and fine-tuning it locally per client. While effective under standard data heterogeneity, where clients share label consensus despite input distribution shifts, this approach struggles under preference heterogeneity, where different clients may assign opposing labels to the same response pair. This fundamental conflict raises a question about whether a single shared initialization can still provide an effective starting point for personalized reward modeling.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.88\textwidth]{fig/fedGD.png}
    \vspace{-9pt}
    \caption{Overview of \alg. \textbf{Phase 1} discovers the preference groups, which can differ in size. \textbf{Phase 2} trains a single reward model over them with group-debiased client sampling, which compensates for group-size imbalance during client selection. The resulting model serves as a shared initialization for personalization. \textbf{Phase 3} personalizes the initial model for each client through a few local optimization steps, yielding \algft.}
    \Description{Three-panel diagram: clients grouped into four preference groups of unequal size, a federated round drawing the same number of clients from every group into one shared model, and that model fine-tuned locally into personalized models.}
    \label{fig:algo}
\end{figure*}

Existing federated methods that explicitly address conflicting preferences or tasks instead avoid this question by clustering similar clients and training one single model per group. For example, FedBiscuit~\citep{wu2024towards} groups clients according to preference similarity, while FedLEASE~\citep{wang2025adaptive} clusters clients across related tasks, so that each client is initialized from a model that never averages over conflicting objectives. However, whether these group-specific initializations actually lead to better personalized reward models than a single shared initialization remains unknown. \textbf{\emph{We therefore ask: what makes a good initialization for personalized reward modeling under preference heterogeneity?}}


% Under preference heterogeneity, no such consensus exists:
% two clients assign opposite labels to the same pair of responses. Federated methods
% facing such conflict, whether from preference or task heterogeneity, cluster similar clients and train one model per group, as
% FedBiscuit~\citep{wu2024towards} does by preference similarity and
% FedLEASE~\citep{wang2025adaptive} does across tasks, so that each client is
% initialized from a model that never had to average over the disagreement. Whether such group-specific initialization is in fact preferable, however, has not been examined on the resulting personalized reward models. We therefore ask what makes a good initialization for personalized reward modeling under preference heterogeneity.


% \newpage



% finding against intuition → mechanism (GQ) → failure under imbalance → FedGD
We find that a group-specific initialization is not the answer. Under balanced preference groups, a single global model trained with FedAvg~\citep{mcmahan2017communication} performs at the level of random guessing before adaptation, yet within a few local steps for personalization, it quickly surpasses both centralized training (CL) and a separate centralized model per ground-truth preference group (Multi-CL).





Our key hypothesis is that preference learning contains two distinct components. The first is \emph{shared knowledge}: identifying the latent feature that distinguishes the two responses. All clients agree on this distinction, so collaborative FL reinforces a common representation of it. The second is \emph{client-specific knowledge}: deciding which side of the latent feature should be preferred. Since this preference differs across clients, no single decision boundary can be optimal for everyone, explaining the poor pre-adaptation accuracy of the global model trained by FL. Consequently, the goal of federated learning should not be to produce the final personalized model, but rather an initialization that captures the shared knowledge while remaining readily adaptable to each client's preference.

To diagnose such an initialization, we adopt the \emph{Gradient Quotient} ($GQ$)~\citep{dauphin2019metainit}, which measures how rapidly the local gradient changes. A small $GQ$ indicates that local optimization remains stable, allowing successive personalization steps to reinforce one another. Such an initialization is therefore well suited for rapidly adapting to each client's local preferences. In our experiments, FedAvg converges to initializations with substantially lower $GQ$ than CL or Multi-CL, which explains why it serves as a better starting point for personalization despite its low start accuracy.

However, when preference groups are imbalanced, the cancellation becomes asymmetric, causing the shared model to become biased toward the majority preferences and reducing its ability to serve as a good initialization for minority clients. We find that balancing client sampling across preference groups during federated training restores the personalization capability of the resulting initialization. By this key observation, we propose \alg\ (\textbf{Fed}erated Learning with \textbf{G}roup \textbf{D}ebiasing), which first discovers the preference groups during FL and then trains a single reward model under group-debiased sampling over the discovered partition (Figure~\ref{fig:algo}).

\textbf{Our contributions are as follows:} 
\begin{itemize}
    \item We introduce an optimization-based perspective on what makes a good initialization for efficient personalization in reward modeling: an initialization
    adapts well when the loss around it is flat, so that successive local steps reinforce one another. We measure this flatness with $GQ$, which tracks how much the local
    gradient changes after a single step.
    
    \item We construct a synthetic benchmark with configurable preference groups and group-size imbalance, enabling controlled analysis for personalized reward modeling under federated settings.
    
    \item We show that, under balanced preference groups, a single FedAvg model provides a better initialization for personalization than both CL and Multi-CL despite its poor
    pre-adaptation accuracy, and identify group imbalance as the condition under which
    this advantage weakens.
    
    \item We propose \alg, which discovers latent preference groups during federated learning and performs group-debiased client sampling to recover high-quality
    initializations without requiring prior knowledge of the true preference groups.
    
\end{itemize}


==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/02_preliminary.tex <==
\section{Preliminaries}
\label{sec:prelim}
We study federated personalized reward modeling, where clients collaboratively train initial global reward models on decentralized pairwise preferences and then fine-tune them locally. We first formalize this workflow (Section~\ref{subsec:fl-procedure}) and then propose two key metrics to evaluate the personalization potential of initial global models (Section~\ref{sec:metrics}). Finally, Section~\ref{sec:ex_design} details the experimental setup.


\subsection{Federated Reward Modeling and Personalization}
\label{subsec:fl-procedure}
We study FL~\cite{mcmahan2017communication} over $C$ clients with pairwise preference data. Each client $c$ holds a local dataset $D_{\text{train}}^c = \{(x_i^c, y_i^{c,+}, y_i^{c,-})\}_{i=1}^{N_c}$, where $x_i^c$ is a prompt, $y_{i}^{c,+}$ the preferred response, and $y_{i}^{c,-}$ the less-preferred one. Let $r_\theta(x, y)$ denote the reward the model assigns to response $y$ for prompt $x$. For a preference $(x, y^{+}, y^{-})$, the \emph{reward margin} $m_\theta(x, y^{+}, y^{-}) = r_\theta(x, y^{+}) - r_\theta(x, y^{-})$ is the signed gap between the two responses, so the prediction is correct when $m_\theta > 0$ and incorrect when $m_\theta \le 0$. Clients minimize the pairwise preference loss $\ell_\theta = -\log \sigma(m_\theta)$, which drives the margin positive, giving the full-batch training loss $\mathcal{L}_c(\theta) = \frac{1}{N_c}\sum_i \ell_\theta(x_i^c, y_i^{c,+}, y_i^{c,-})$ of client $c$.

FL proceeds over $R$ communication rounds.
At the beginning of round $r$, the server broadcasts the current global parameters $\theta^{(r-1)}$ to a sampled subset of clients $S_r \subset [C]$.
Each selected client $c \in S_r$ performs $\tau$ local training iterations on $D_{\text{train}}^c$ with batch size $B$, and returns updated parameters $\theta_{c}^{(r)}$.
The server aggregates these local updates via weighted averaging~\cite{li2019convergence, wu2024towards} to obtain the new global parameters $\theta^{(r)}$. The description above corresponds to a single-global design in which the server maintains a single parameter vector $\theta^{(r)}$. Some of the designs we compare instead maintain $K$ global models $\{\theta_k^{(r)}\}_{k=1}^K$ on the server and apply the same broadcast--update--aggregate procedure independently to each model over its associated subset of clients.

After $R$ training rounds in the \emph{global} phase, we run a separate \emph{personalization} phase. Each client $c$ receives a single initialization $\theta_c^{\text{init}}$, fine-tunes it on its own preference data $D_{\text{train}}^c$ without further communication, and obtains a personalized reward model $\theta_c^{\text{PFL}}$. Since local adaptation runs on the client, where compute is limited, the number of local steps an initialization requires is itself a cost. We therefore report accuracy after a small number of local steps alongside the accuracy eventually reached. How $\theta_c^{\text{init}}$ is constructed is the design choice we study, and we specify it for each method in Sections~\ref{sec:motivation} and~\ref{sec:exp}. Throughout the paper, we refer to the models that serve as initializations for personalization as \emph{global} models and to $\theta_c^{\text{PFL}}$ as the resulting \emph{personalized} reward model for client $c$.

\subsection{Quantifying Personalization Capability}
\label{sec:metrics}
Given a reward model $\theta$ as the \emph{initialization} for
personalization, we characterize its personalization capability by estimating how effectively a small number of local updates can improve it. For this, we introduce two diagnostics: (i) \emph{Gradient Quotient} ($GQ$)~\cite{dauphin2019metainit}, a model-level measure of \emph{flatness} that assesses whether consecutive local steps reinforce one another, and (ii) \emph{Headroom} ($H$), a per-sample measure that we propose to assess whether a local update moves an individual sample toward its correct preference. Both quantities are computed using each client's local preference data.

% \smallskip
\noindent\textbf{Gradient Quotient ($GQ$): flatness of the initialization.}\quad 
A good initialization should be one from which local updates consistently move toward the client's optimum rather than changing gradient dramatically after one update. We measure this property using the $GQ$~\cite{dauphin2019metainit}, which quantifies how much the gradient changes after a single optimization step.

Let
$g^c(\theta) = \nabla \mathcal{L}_c(\theta)$ be the gradient of client $c$'s
full-batch training loss and $g^{c,l}$ its restriction to the LoRA parameters
$\theta^l$ of layer $l$. The layer-wise $GQ$ is
\begin{align*}
GQ(c, l)
&= \frac{1}{\#\theta^l}
\left\lVert \frac{g^{c,l}\!\big(\theta - \eta\, g^c(\theta)\big)}{g^{c,l}(\theta)} - \mathbf{1} \right\rVert_1
\approx
\frac{\eta}{\#\theta^l}
\left\lVert \frac{[\nabla^2\mathcal{L}_c(\theta)\, g^c(\theta)]^{\,l}}{g^{c,l}(\theta)} \right\rVert_1 ,
\end{align*}
where $\#\theta^l$ is the number of LoRA parameters in layer $l$. The first-order
approximation shows that $GQ$ is determined by the Hessian–gradient product, which captures the local curvature along the update direction. Consequently, $GQ$ increases with the curvature encountered by gradient descent. A small $GQ$ indicates that the gradient remains nearly unchanged in both direction and magnitude, allowing successive local updates to remain aligned and accumulate toward the client's optimum. In contrast, a large $GQ$ indicates that the gradient is rapidly distorted after a single step, causing subsequent steps to deviate from the original descent direction and partially cancel earlier progress, thereby reducing the effectiveness of local personalization.

We obtain a layer-wise statistic by averaging over clients,
$GQ(l) = \tfrac{1}{C}\sum_c GQ(c, l)$ over the $24$ LoRA-adapted layers of
Qwen2-0.5B~\cite{yang2024qwen2technicalreport}, our base model
(Section~\ref{sec:exp}). Studies of few-step adaptation commonly separate a
shared representation body from task-specific upper layers, both in
meta-learning~\cite{oh2021boil} and in personalized FL~\cite{oh2021fedbabu}, so we
report a Body average $GQ_{\mathcal{B}}$ over the front $16$ layers and a Head
average $GQ_{\mathcal{H}}$ over the back $8$.


\noindent\textbf{Headroom ($H$): one-step correctability of a sample.}\quad
$GQ$ measures whether local updates are stable, not whether they lead to
the right direction. We define \emph{Headroom} to answer the latter for a single
sample. Starting from the initialization under evaluation,
$\theta_0 = \theta_c^{\text{init}}$, we take one full-batch \emph{training} step on
client $c$'s data, $\theta_1 = \theta_0 - \eta\, g^{c}(\theta_0)$, and define the
Headroom as the first-order effect of this step on the margin of a held-out
\emph{test} sample $(x, y^{+}, y^{-})$ of the same client:
\begin{equation*}
H(x, y^{+}, y^{-})
= -\eta\, \big\langle \nabla_\theta m_\theta\big|_{\theta_0},\ g^{c}(\theta_0) \big\rangle
\approx \Delta m,
\end{equation*}
where $\Delta m = m_{\theta_1} - m_{\theta_0}$ is the true margin change. A
positive $H$ means one training step moves the held-out sample toward its correct
preference, and a larger $H$ indicates more room to move it.

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{0.95}
\caption{Diagnostics and personalized accuracy under balanced settings. $GQ(l)$: mean$\pm$std over the 24 layers, with Body/Head averages $GQ_{\mathcal{B}}, GQ_{\mathcal{H}}$. $\mathcal{R}$ / $\mathcal{W}$: test samples initially correct / wrong at $\theta_0$. $m^{0}$: mean reward margin at $\theta_0$. $H^{+}$: fraction with positive Headroom. $P^{10}$: fraction correct after 10 local steps. $\mathrm{acc}^{0}$ in parentheses. Highlighting the best $\mathrm{acc}^{10}$ and bold the best per column.}
\label{tab:balanced}
\vspace{-8pt}
\begin{tabular}{lccc cc cc cc c}
\toprule
& \multicolumn{3}{c}{Flatness ($\downarrow$)}
& \multicolumn{2}{c}{Margin ($m^{0}$)}
& \multicolumn{2}{c}{Retention ($\mathcal{R}$, \%, $\uparrow$)}
& \multicolumn{2}{c}{Correction ($\mathcal{W}$, \%, $\uparrow$)}
& \multicolumn{1}{c}{Accuracy (\%, $\uparrow$)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
method & $GQ(l)$ & $GQ_{\mathcal{B}}$ & $GQ_{\mathcal{H}}$
       & $m^{0}_{\mathcal{R}}$ & $m^{0}_{\mathcal{W}}$
       & $H^{+}_{\mathcal{R}}$ & $P^{10}_{\mathcal{R}}$
       & $H^{+}_{\mathcal{W}}$ & $P^{10}_{\mathcal{W}}$
       & $\mathrm{acc}^{10}\,(\mathrm{acc}^{0})$ \\
\midrule
CL       & $1.14 \pm 0.24$ & 1.29 & 0.84
         & $+16.00$ & $-15.77$
         & 34.18 & 82.32 & 62.02 & 21.49
         & 52.15 (50.45) \\
Multi CL & $0.86 \pm 0.23$ & 1.00 & 0.56
         & $+22.88$ & $-12.39$
         & 13.01 & \textbf{97.28} & 59.51 & 25.77
         & 91.45 (92.20) \\
\rowcolor{flhl}
FL       & $\mathbf{0.10 \pm 0.01}$ & \textbf{0.11} & \textbf{0.09}
         & $+2.38$ & $-2.34$
         & \textbf{56.94} & 94.01 & \textbf{96.00} & \textbf{91.99}
         & \textbf{93.45 (50.40)} \\
\bottomrule
\end{tabular}
\end{table*}



We compute $H$ for every sample in the client's held-out test split. Since
correctability depends on whether a sample is already correct, we partition the
test set at $\theta_0$ into the \emph{retention} set $\mathcal{R} = \{m_{\theta_0} > 0\}$
and the \emph{correction} set $\mathcal{W} = \{m_{\theta_0} \le 0\}$, and report for
each set the mean Headroom $H^{0}$ and the fraction of samples with positive
Headroom $H^{+}$, averaged over clients.


\subsection{Datasets and Preference Groups}
\label{sec:ex_design}
We evaluate on two datasets: a real-world set with natural annotator preferences, and a synthetic set with controlled style heterogeneity. For each client, we reserve 50 samples each for validation and testing, and use the rest for training.


\noindent\textbf{Real-world dataset.}\quad
We use the Reddit TL;DR summarization dataset~\citep{stiennon2020learning, volske2017tl}, which contains human preference annotations along with client IDs. We filter 144,502 samples for 34 clients who participate in all three train/valid1/valid2 splits with at least 100 samples each. Each client corresponds to an actual human annotator, and the dataset inherently exhibits natural data imbalance and genuine preference heterogeneity, with the underlying preference groups being \emph{unknown}.

\noindent\textbf{Synthetic dataset.}\quad
We gather prompts by combining UltraFeedback~\citep{cui2023ultrafeedback} and p-Soups~\citep{jang2023personalized}, resulting in 52K unique prompts. Using GPT-4o-mini,\footnote{\url{https://platform.openai.com/docs/models/gpt-4o-mini}}we generate two candidate responses per prompt along two style axes---(1) \emph{Elementary} vs.\ \emph{PhD-level} and (2) \emph{Humorous} vs.\ \emph{Non-humorous}---allocating 26K prompts per axis. We then simulate 40 clients (650 samples per axis), grouped into the four preference groups formed by the two axes: (G1) Elementary/Humorous, (G2) Elementary/Non-humorous, (G3) PhD/Humorous, and (G4) PhD/Non-humorous. Clients are indexed by group, starting with G1 and progressing through G4 in sequence.


% \smallskip
\noindent\textbf{Group-size balance.}\quad
Using the synthetic dataset, we evaluate how effectively the initial shared model adapts to individual clients under varying group-size distributions. We consider two group-size configurations across G1, G2, G3, and G4:
\begin{itemize}\setlength\itemsep{1pt}
    \item \textbf{Balanced (10/10/10/10):} 10 clients per group, maintaining an equal balance across both preference axes.
    \item \textbf{Imbalanced (15/15/5/5):} the Elementary-dominant groups (G1, G2) are overrepresented while the PhD-dominant groups (G3, G4) are underrepresented, naturally biasing the shared model toward the majority preference.
\end{itemize}




==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/03_motivation.tex <==
% \begin{table*}[t]
% \centering
% \caption{Diagnostics and personalized accuracy under the balanced setting.
% $GQ(l)$ is the mean$\pm$std over the 24 layers, with its Body and Head averages
% $GQ_{\mathcal{B}}, GQ_{\mathcal{H}}$. For the retention set $\mathcal{R}$
% (initially correct) and the correction set $\mathcal{W}$ (initially wrong)
% defined in Section~\ref{sec:metrics}, $H^{+}$ is the fraction of samples with
% positive Headroom and $P^{10}$ the fraction answered correctly after 10 local
% steps. $\mathrm{acc}^{10}$ is the overall accuracy after 10 steps, with
% $\mathrm{acc}^{0}$ at initialization in parentheses. Highlighting marks the best
% $\mathrm{acc}^{10}$; bold marks the best value per column.}
% \label{tab:balanced}
% \vspace{-8pt}
% \begin{tabular}{lccc cc cc c}
% \toprule
% & \multicolumn{3}{c}{Flatness ($\downarrow$)}
% & \multicolumn{2}{c}{Retention ($\mathcal{R}$, \%, $\uparrow$)}
% & \multicolumn{2}{c}{Correction ($\mathcal{W}$, \%, $\uparrow$)}
% & \multicolumn{1}{c}{Accuracy (\%, $\uparrow$)} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9}
% method & $GQ(l)$ & $GQ_{\mathcal{B}}$ & $GQ_{\mathcal{H}}$
%        & $H^{+}_{\mathcal{R}}$ & $P^{10}_{\mathcal{R}}$
%        & $H^{+}_{\mathcal{W}}$ & $P^{10}_{\mathcal{W}}$
%        & $\mathrm{acc}^{10}\,(\mathrm{acc}^{0})$ \\
% \midrule
% % Base     & $0.48 \pm 0.01$ & 0.48 & 0.48 & 0.81  & 94.81 & 99.31 & 5.30  & 49.25 (49.10) \\
% CL       & $1.14 \pm 0.24$ & 1.29 & 0.84 & 34.18 & 82.32 & 62.02 & 21.49 & 52.15 (50.45) \\
% Multi CL & $0.86 \pm 0.23$ & 1.00 & 0.56 & 13.01 & \textbf{97.28} & 59.51 & 25.77 & 91.45 (92.20) \\
% \rowcolor{flhl}
% FL       & $\mathbf{0.10 \pm 0.01}$ & \textbf{0.11} & \textbf{0.09}
%          & \textbf{56.94} & 94.01 & \textbf{96.00} & \textbf{91.99}
%          & \textbf{93.45 (50.40)} \\
% \bottomrule
% \end{tabular}
% \end{table*}

\section{A Single Federated Model Suffices, Until Group Imbalance}
\label{sec:motivation}

In this section, we compare three initializations in terms of the personalization capability of the resulting models. Interestingly, our finding indicates that FL provides a stronger initialization when preference groups are well balanced. Results show that this advantage arises because the local training loss is relatively flat around the initialization, while most test samples retain positive Headroom toward the correct preference. However, this benefit weakens under group imbalance, where FL becomes increasingly biased toward majority preferences and adaptation slows sharply. These findings motivate \alg, our proposed approach.

% \smallskip
\noindent\textbf{Compared initializations.}\quad
We compare 3 ways of producing the reward model that each client fine-tunes locally, trained for 200 communication rounds with the same number of updates.

\begin{itemize}
\setlength\itemsep{2pt}
    \item \textbf{CL:} pools all preference data on one server and trains a single centralized model, so conflicting preferences are mixed \emph{within every batch}.
    \item \textbf{FL:} trains a single global model with FedAvg~\cite{mcmahan2017communication}, so the conflict is concentrated
    \emph{at aggregation}.
    \item \textbf{Multi-CL:} trains one centralized model per ground-truth preference group, so \emph{no conflict arises within a model}. Each client is initialized from its own group's model. Since the true groups are unknown in practice, Multi-CL is a reference point rather than a deployable method.
\end{itemize}


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{fig/groupwise_balance_steps0_80_by10_with_legend.pdf}
    \vspace{-12pt}
    \caption{Group-wise personalized accuracy under the balanced setting, evaluated every 10 steps up to 80 local fine-tuning steps.}
    \Description{}
    \label{fig:groupwise_balance}
\end{figure}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{0.95}
\caption{Diagnostics and personalized accuracy under the imbalanced setting
(15/15/5/5); the first row repeats balanced FL for reference.
$GQ(l)$: mean$\pm$std over the 24 LoRA layers, with Body/Head averages
$GQ_{\mathcal{B}}, GQ_{\mathcal{H}}$. $\mathcal{R}$ / $\mathcal{W}$: test
samples initially correct / wrong at $\theta_0$. $m^{0}$: mean reward margin
at $\theta_0$. $H^{+}$: fraction with positive headroom. $P^{10}$: fraction
correct after 10 local steps. Highlighting marks the best
$\mathrm{acc}^{10}$; bold the best per column among the imbalanced rows.}
\label{tab:imbalanced}
\vspace{-8pt}
\begin{tabular}{lccc cc cc cc c}
\toprule
& \multicolumn{3}{c}{Flatness ($\downarrow$)}
& \multicolumn{2}{c}{Margin ($m^{0}$)}
& \multicolumn{2}{c}{Retention ($\mathcal{R}$, \%, $\uparrow$)}
& \multicolumn{2}{c}{Correction ($\mathcal{W}$, \%, $\uparrow$)}
& \multicolumn{1}{c}{Accuracy (\%, $\uparrow$)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
method & $GQ(l)$ & $GQ_{\mathcal{B}}$ & $GQ_{\mathcal{H}}$
       & $m^{0}_{\mathcal{R}}$ & $m^{0}_{\mathcal{W}}$
       & $H^{+}_{\mathcal{R}}$ & $P^{10}_{\mathcal{R}}$
       & $H^{+}_{\mathcal{W}}$ & $P^{10}_{\mathcal{W}}$
       & $\mathrm{acc}^{10}\,(\mathrm{acc}^{0})$ \\
\midrule
\rowcolor{flhl}
FL (balanced) & $0.10 \pm 0.01$ & 0.11 & 0.09
              & $+2.38$ & $-2.34$
              & 56.94 & 94.01 & 96.00 & 91.99
              & 93.45 (50.40) \\
\midrule
CL         & $1.09 \pm 0.28$ & 1.25 & 0.76
           & $+20.41$ & $-19.42$
           & 25.72 & 86.50 & 69.61 & 20.14
           & 60.50 (59.85) \\
Multi CL   & $0.95 \pm 0.25$ & 1.11 & 0.63
           & $+23.96$ & $-11.79$
           & 10.44 & 97.60 & 58.42 & 26.14
           & 91.50 (92.10) \\
FL         & $0.72 \pm 0.25$ & 0.88 & 0.39
           & $+27.90$ & $-27.02$
           & 3.08 & \textbf{99.11} & \textbf{96.74} & 2.09
           & 61.75 (61.80) \\
\rowcolor{fthl}
FL\_target & $\mathbf{0.27 \pm 0.02}$ & \textbf{0.28} & \textbf{0.24}
           & $+3.59$ & $-3.65$
           & \textbf{75.78} & 93.42 & 93.44 & \textbf{90.62}
           & \textbf{92.35 (54.95)} \\
\bottomrule
\end{tabular}
\end{table*}



% \vspace{-5pt}
\subsection{FL Suffices Under Balanced Groups}
\label{sec:motivation-balanced}
Under the balanced setting, FL shows the best initialization for personalization. Let $\mathrm{acc}^{0}$ denote the accuracy of an initialization before any local update and $\mathrm{acc}^{10}$ the accuracy after 10 local fine-tuning steps, both averaged over clients. Before fine-tuning, Multi-CL reaches $\mathrm{acc}^{0} = 92.20$, while CL and FL reach only $50.45$ and $50.40$, the accuracy of random guessing on binary preference pairs (Table~\ref{tab:balanced}). Figure~\ref{fig:groupwise_balance} shows that this average hides a wide spread for FL, whose initial accuracy ranges from about $20\%$ on G2 to about $80\%$ on G3. However, just 10 local steps change the picture: FL reaches $\mathrm{acc}^{10} = 93.45$ and overtakes Multi-CL, which ends at $91.45$, slightly below where it started, while CL improves only to $52.15$. The same pattern appears in every group: FL gains almost all of its improvement within 10 steps, whereas CL improves only gradually over 80 steps and Multi-CL changes little or slightly declines.

% FL gains the most from a few local steps despite a low initial accuracy. Table \ref{tab:balanced} indicates that the phenomenon is because the
% loss around the FL model is flat across all layers. Every client must detect the
% style axis to fit its own labels, and what differs is only which side each client
% prefers, so averaging the locally trained models reinforces the shared detection
% while the opposing choices offset. CL admits no separation between detecting the
% axis and choosing a side, since conflicting preferences enter the same batch.
% Multi-CL removes the conflict but trains each model on a quarter of the clients, all
% sharing one preferred direction, so the axis is learned from less diverse data. FL
% accordingly keeps the Body and the Head at nearly the same level
% ($GQ_{\mathcal{B}} = 0.11$, $GQ_{\mathcal{H}} = 0.09$), whereas CL and Multi-CL are
% sharper throughout and most so in the Body ($GQ_{\mathcal{B}} = 1.29$ and $1.00$),
% the layers that detect the axis.

FL gains the most from a few local steps despite its low initial accuracy, and
Table~\ref{tab:balanced} attributes this to a loss that is flat across all layers
around the FL model. The flatness follows from how far each initialization has
already committed. Every client must detect what distinguishes the two responses---here the style axis---to fit its own labels, and what differs is only which side it prefers, so averaging the locally trained models reinforces the shared detection while the opposing side choices offset one another. The resulting model therefore sits close to the decision boundary, with initial margins of only $m^{0}_{\mathcal{R}} = +2.38$ and
$m^{0}_{\mathcal{W}} = -2.34$, where the loss $-\log\sigma(m)$ is far from
saturation and its gradient changes slowly. CL cannot separate detecting the axis
from choosing a side, since conflicting preferences enter the same batch, and
Multi-CL removes the conflict entirely by training each model on a quarter of the
clients that share one direction; both commit to a side and reach
$m^{0}_{\mathcal{R}} = +16.00$ and $+22.88$, deep in the saturated regime where a
single step distorts the gradient. This is reflected in the diagnostics: FL is an
order of magnitude flatter than both baselines at every layer
($GQ_{\mathcal{B}} = 0.11$ vs.\ $1.29$ and $1.00$; $GQ_{\mathcal{H}} = 0.09$
vs.\ $0.84$ and $0.56$), and the gap is largest in the Body, the layers that
detect the axis.

On the flat FL initialization, fine-tuning corrects wrong predictions without
sacrificing the correct ones. For FL, $96.00\%$ of the wrong set $\mathcal{W}$
carries positive headroom ($H^{+}_{\mathcal{W}}$), and after 10 steps $91.99\%$ of
$\mathcal{W}$ is answered correctly ($P^{10}_{\mathcal{W}}$), while $94.01\%$ of
the right set $\mathcal{R}$ stays correct ($P^{10}_{\mathcal{R}}$). CL and Multi-CL
start with less headroom on $\mathcal{W}$ ($62.02\%$ and $59.51\%$) and correct
only $21.49\%$ and $25.77\%$ of it, even though Multi-CL keeps slightly more of
$\mathcal{R}$ than FL ($97.28\%$).

\vspace{-10pt}
\subsection{Group-Debiased Sampling Restores FL Under Imbalance}
\label{sec:motivation-imbalanced}
Under group imbalance, FL adapts more slowly. Although FL begins with a substantially higher accuracy than in the balanced case, 10 local steps leave it essentially unchanged. FL starts in $\mathrm{acc}^{0} = 61.80$, compared with $50.40$ under balanced groups, yet reaches only $\mathrm{acc}^{10} = 61.75$~(Table~\ref{tab:imbalanced}). Figure~\ref{fig:groupwise_imbalance} shows that the initial accuracy again varies widely across groups, from near $10\%$ on G4 to $98\%$ on G1, but the gains from fine-tuning are smaller than under balanced groups, where every group rose above $90\%$ within 10 steps. G2, G3, and G4 instead climb slowly and stay below G1 even after 80 steps.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/groupwise_imbalance_steps0_80_by10_with_legend.pdf}
    \vspace{-8pt}
    \caption{Group-wise PFL accuracy under the imbalanced setting for the four methods (CL, Multi CL, FL, and FL\_target), evaluated every 10 steps up to 80 fine-tuning steps.}
    \label{fig:groupwise_imbalance}
\end{figure}

% \begin{table*}[t]
% \centering
% \caption{Diagnostics and personalized accuracy under the imbalanced setting
% (15/15/5/5). $GQ(l)$ is reported as mean$\pm$std over the 24 layers, with its Body
% and Head averages. Accuracy after 10 local steps is given with the initial accuracy
% in parentheses. Highlighting marks the best $\mathrm{acc}^{10}$ in each setting,
% and bold marks the best value per column within the imbalanced setting.}
% \label{tab:imbalanced}
% \vspace{-8pt}
% \begin{tabular}{llccc cc cc c}
% \toprule
% & & \multicolumn{3}{c}{Flatness ($\downarrow$)}
% & \multicolumn{2}{c}{Retention ($\mathcal{R}$, \%, $\uparrow$)}
% & \multicolumn{2}{c}{Correction ($\mathcal{W}$, \%, $\uparrow$)}
% & \multicolumn{1}{c}{Accuracy (\%, $\uparrow$)} \\
% \cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-10}
% setting & method & $GQ(l)$ & $GQ_{\mathcal{B}}$ & $GQ_{\mathcal{H}}$
%         & $H^{+}_{\mathcal{R}}$ & $P^{10}_{\mathcal{R}}$
%         & $H^{+}_{\mathcal{W}}$ & $P^{10}_{\mathcal{W}}$
%         & $\mathrm{acc}^{10}\,(\mathrm{acc}^{0})$ \\
% \midrule
% \rowcolor{flhl}
% Balanced & FL & $0.10 \pm 0.01$ & 0.11 & 0.09 & 56.94 & 94.01 & 96.00 & 91.99
%          & 93.45 (50.40) \\
% \midrule
% Imbalanced & CL          & $1.09 \pm 0.28$ & 1.25 & 0.76 & 25.72 & 86.50 & 69.61 & 20.14 & 60.50 (59.85) \\
% Imbalanced & Multi CL    & $0.95 \pm 0.25$ & 1.11 & 0.63 & 10.44 & \textbf{97.60} & 58.42 & 26.14 & 91.50 (92.10) \\
% Imbalanced & FL          & $0.72 \pm 0.25$ & 0.88 & 0.39 & 3.08 & 99.11 & \textbf{96.74} & 2.09 & 61.75 (61.80) \\
% \rowcolor{fthl}
% Imbalanced & FL\_target  & $\mathbf{0.27 \pm 0.02}$ & \textbf{0.28} & \textbf{0.24} & \textbf{75.78} & 93.42 & 93.44 & \textbf{90.62} & \textbf{92.35 (54.95)} \\
% \bottomrule
% \end{tabular}
% \end{table*}

To test the hypothesis that the degradation in personalization is caused by group imbalance rather than the FL procedure itself, we consider a group-debiased sampling strategy that prevents any preference group from being underrepresented in a communication round. Specifically, we modify FL only in the client sampling step while leaving the rest of the training procedure unchanged, denoted by FL\_target. In our experiments, each round samples $|S_r| = 5$ clients: one from each of the four groups and one additional client chosen uniformly at random from all groups. This simple modification lifts accuracy from $\mathrm{acc}^{0} = 54.95$ to $\mathrm{acc}^{10} = 92.35$, a level standard FL does not reach within the same number of local steps ($\mathrm{acc}^{0} = 61.80$ to $\mathrm{acc}^{10} = 61.75$) (Table~\ref{tab:imbalanced}). Figure~\ref{fig:groupwise_imbalance} shows FL\_target exceeding $90\%$ on every group within 10 local steps, a behavior FL showed only in the balanced setting. On this dataset, \alg\ with $K=4$ recovers the four ground-truth groups exactly, so FL\_target coincides with \alg\ (Section~\ref{sec:method}). 

Group-debiased sampling works by keeping the loss uniformly flat across layers,
unlike uniform sampling. Under FL, the Body degrades far more than the Head, with
$GQ_{\mathcal{B}}$ rising from $0.11$ in the balanced setting to $0.88$ and
$GQ_{\mathcal{H}}$ from $0.09$ to $0.39$ (Table~\ref{tab:imbalanced}). Correction
suffers as well: $96.74\%$ of the wrong set $\mathcal{W}$ still carries positive
headroom, yet only $2.09\%$ of $\mathcal{W}$ is answered correctly after 10 steps,
against $91.99\%$ in the balanced setting. The direction of the update is therefore right but its reach is not: imbalanced FL
commits to the majority side and starts at $m^{0}_{\mathcal{W}} = -27.02$, an
order of magnitude beyond the balanced case ($-2.34$), so ten steps cannot close
the gap. The right set $\mathcal{R}$ changes little instead, with $99.11\%$ staying correct but only $3.08\%$ carrying positive headroom. FL\_target starts lower than FL at $\mathrm{acc}^{0} = 54.95$, yet keeps
the Body and the Head close ($GQ_{\mathcal{B}} = 0.28$, $GQ_{\mathcal{H}} = 0.24$) and stays near the decision
boundary ($m^{0}_{\mathcal{W}} = -3.65$ against $-27.02$ for FL), raises $H^{+}_{\mathcal{R}}$ from $3.08\%$ to $75.78\%$, and recovers correction to
$P^{10}_{\mathcal{W}} = 90.62\%$. Group-debiased sampling is therefore what lets FL adapt within a few local steps
under group imbalance. However, FL\_target assumes access to the true preference groups, which are unknown in practice.
This naturally raises the following question: \emph{``Can group debiasing be achieved without knowing the true preference groups?''}

==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/04_method.tex <==
\section{Federated Learning with Group Debiasing}
\label{sec:method}
In this section, we propose \alg, which applies group debiasing when the true groups
are unknown. \alg proceeds in two phases: (1) discovering the groups during
federated learning, and (2) training a single reward model with group-debiased
sampling over the discovered groups. Each client then fine-tunes the resulting
model following the personalization phase of Section~\ref{subsec:fl-procedure},
yielding the personalized reward models we denote by \algft. The full algorithm is
given in Appendix~\ref{app:fedgd}.

\input{tables/pfl}

\subsection{Phase 1: Discovering the Groups}
We discover the groups with clustered FL~\cite{ghosh2020efficient, sattler2020clustered},
which partitions clients by training several models and letting each client join the
one that fits its data best. Over the first $R/2$ rounds, the server maintains $K$
expert models $\{\theta_k\}_{k=1}^{K}$ together with a reference model $\theta_g$,
and each client is assigned to one expert, forming the groups
$\{\mathcal{A}_k\}_{k=1}^{K}$. Every $T$ rounds the clients are reassigned, and in
the rounds between two reassignments the experts are trained on the clients
currently assigned to them. After round $R/2$ the clients are reassigned once more,
and the resulting groups $\{\mathcal{A}_k^{\star}\}_{k=1}^{K}$ are frozen; empty
clusters are discarded, so $K$ denotes the number of discovered groups. Neither the
experts nor $\theta_g$ is used as an initialization for personalization; they serve
only to discover the groups.

% \smallskip
\noindent\textbf{Reassigning clients ($\pi(c)$).}\quad
Clients start from a uniform random assignment. Every $T$ rounds each client
evaluates all $K$ experts on its own validation split and is reassigned to the
expert with the lowest validation loss~\cite{wu2024towards},
\begin{equation*}
\pi(c) \leftarrow \arg\min_{k} \operatorname{ValLoss}(\theta_k, D^c_{\text{val}}),
\qquad
\mathcal{A}_k = \{c : \pi(c) = k\},
\end{equation*}
where $\pi(c)$ denotes the expert assigned to client $c$. Each reassignment also
resets every expert to the current reference model, $\theta_k \leftarrow \theta_g$,
so that the experts do not inherit what they learned from the clients they had
before.

% \smallskip
\noindent\textbf{Updating the reference model ($\theta_g$).}\quad
Each round draws clients with group-debiased sampling over the current groups
$\{\mathcal{A}_k\}_{k=1}^{K}$. Specifically, clients are sampled from each group with probability inversely proportional to the group's cardinality, so that the resulting client set has a uniform group composition regardless of group size. We denote the resulting participating set $G_r$, the
\textit{group-debiased} counterpart of the sampled set $S_r$ of
Section~\ref{subsec:fl-procedure}. The reference model averages the returned models
uniformly,
\begin{equation*}
\theta_g^{(r)} = \frac{1}{|G_r|} \sum_{c \in G_r} \theta^{(r)}_{\pi(c), c}.
\end{equation*}
Here $\theta_g$ serves as a neutral point to which the experts are reset rather
than as a loss minimizer, and every client takes the same $\tau$ local steps, so
weighting by dataset size would bias the discovered partition toward data volume
rather than preference.

% \smallskip
\noindent\textbf{Training the experts ($\theta_k$).}\quad
Every selected client $c \in G_r$ receives the expert $\theta_{\pi(c)}^{(r-1)}$ of its
own group, trains it on its local data, and returns the updated model
$\theta^{(r)}_{\pi(c), c}$ to the server. To estimate each expert from more than the
clients of a single round, the server accumulates the returned models and takes
their cumulative average,
\begin{equation*}
s_k = \frac{1}{n_k} \sum_{r'=r_0}^{r} \sum_{c \in G_{r'} \cap \mathcal{A}_k}
\theta^{(r')}_{k, c},
\qquad
n_k = \sum_{r'=r_0}^{r} |G_{r'} \cap \mathcal{A}_k|,
\end{equation*}
where $r_0$ is the round of the last reassignment. The expert is then updated as a
moving average of its previous value and $s_k$,
\begin{equation*}
\theta_k^{(r)} = (1-w)\, \theta_k^{(r-1)} + w\, s_k .
\end{equation*}

% \subsection{Phase 2: Training the Reward Model}
% The remaining $R/2$ rounds train a single reward model $\phi$ with group-debiased
% sampling over the frozen groups $\{\mathcal{A}_k^{\star}\}_{k=1}^{K}$, starting from
% a randomly initialized $\phi^{(0)}$. Each selected client $c \in G_r$ trains
% $\phi^{(r)}$ on its local data and returns $\phi^{(r+1)}_c$, and the server
% aggregates the returned models in proportion to the local dataset sizes $N_c$,
% \begin{equation*}
% \phi^{(r+1)} = \sum_{c \in G_r} \frac{N_c}{\sum_{c' \in G_r} N_{c'}}\, \phi^{(r+1)}_c .
% \end{equation*}
% The resulting $\phi^{(R)}$ is the single global model that every client
% personalizes; note that $\phi$ is trained for only $R/2$ rounds, half the budget
% given to the baselines.

\subsection{Phase 2: Training the Reward Model}
The remaining $R/2$ rounds train a single reward model $\phi$ over the frozen
groups $\{\mathcal{A}_k^{\star}\}_{k=1}^{K}$, starting from a randomly
initialized $\phi^{(R/2)}$. Each round draws clients with group-debiased sampling
and each selected client trains $\phi^{(r)}$ on its local data, returning
$\phi^{(r+1)}_c$. Write $G^{\star}_{r,k}$ for the clients of group $k$ that
participate in round $r$.

Aggregation is \emph{hierarchical}: size-weighted within a group, uniform
across groups:
\begin{equation*}
\bar\phi^{(r+1)}_k
= \sum_{c \in G^{\star}_{r,k}}
  \frac{N_c}{\sum_{c' \in G^{\star}_{r,k}} N_{c'}}\, \phi^{(r+1)}_c ,
\qquad
\phi^{(r+1)}
= \frac{1}{|\mathcal{K}_r|} \sum_{k \in \mathcal{K}_r} \bar\phi^{(r+1)}_k ,
\end{equation*}
where $\mathcal{K}_r$ indexes the groups reached in round $r$. Each group
contributes one model regardless of its size, so the debiasing applied at
sampling is preserved at aggregation.

The resulting $\phi^{(R)}$ is the initial global model from which every client
personalizes using its own local preference data.

==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/05_exp.tex <==
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{PFL accuracy comparison, reported as mean$_{\pm\text{std}}$ over
% clients from a single seed. $\mathrm{acc}^{t}$: accuracy after $t$ local
% fine-tuning steps. Multi CL requires known groups and is not deployable on
% real annotators (``--''). \textbf{Bold} marks the best value in each
% post-adaptation column.}
% \label{tab:pfl}
% \vspace{-8pt}
% \begin{tabular}{l ccc ccc ccc}
% \toprule
% & \multicolumn{3}{c}{Balanced (Synthetic)}
% & \multicolumn{3}{c}{Imbalanced (Synthetic)}
% & \multicolumn{3}{c}{Real-world} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% Algorithm & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{10}$ & $\mathrm{acc}^{80}$
%           & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{10}$ & $\mathrm{acc}^{80}$
%           & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{80}$ & $\mathrm{acc}^{240}$ \\
% \midrule
% Base
%   & $\acc{49.20}{6.97}$ & $\acc{49.95}{7.26}$ & $\acc{58.05}{7.69}$
%   & $\acc{50.25}{7.27}$ & $\acc{51.30}{7.44}$ & $\acc{58.70}{7.07}$
%   & $\acc{51.24}{6.84}$ & $\acc{52.12}{6.65}$ & $\acc{54.59}{7.66}$ \\
% \addlinespace[2pt]
% CL
%   & $\acc{51.80}{7.48}$ & $\acc{53.70}{7.15}$ & $\acc{55.40}{5.99}$
%   & $\acc{56.00}{11.86}$ & $\acc{56.90}{10.89}$ & $\acc{62.60}{7.93}$
%   & $\acc{58.06}{7.81}$ & $\acc{57.06}{9.08}$ & $\acc{61.00}{6.69}$ \\
% Multi CL
%   & $\acc{92.10}{4.02}$ & $\acc{92.15}{3.88}$ & $\acc{91.60}{4.29}$
%   & $\acc{92.30}{3.42}$ & $\acc{91.70}{3.63}$ & $\acc{91.60}{3.67}$
%   & -- & -- & -- \\
% FL~\cite{mcmahan2017communication}
%   & $\acc{50.35}{23.15}$ & $\acc{92.45}{3.76}$ & $\mathbf{\acc{94.70}{2.92}}$
%   & $\acc{55.60}{21.36}$ & $\acc{90.55}{5.20}$ & $\mathbf{\acc{93.80}{3.40}}$
%   & $\acc{60.82}{7.75}$ & $\acc{61.53}{7.70}$ & $\acc{63.00}{9.10}$ \\
% \addlinespace[2pt]
% FedBiscuit~\cite{wu2024towards}
%   & $\acc{68.80}{9.76}$ & $\acc{66.90}{6.18}$ & $\acc{71.45}{10.35}$
%   & $\acc{78.45}{10.54}$ & $\acc{77.85}{9.85}$ & $\acc{80.80}{8.46}$
%   & $\acc{57.35}{6.80}$ & $\acc{58.47}{7.96}$ & $\acc{57.24}{6.88}$ \\
% Soft-FL (ours)
%   & $\acc{51.70}{9.43}$ & $\acc{62.40}{7.51}$ & $\acc{71.30}{6.09}$
%   & $\acc{56.50}{13.67}$ & $\acc{75.95}{9.81}$ & $\acc{86.20}{7.41}$
%   & $\acc{59.94}{6.41}$ & $\acc{59.00}{8.59}$ & $\acc{59.00}{7.58}$ \\
% FedGD (ours)
%   & $\acc{49.15}{13.45}$ & $\mathbf{\acc{94.55}{3.58}}$ & $\acc{94.30}{3.86}$
%   & $\acc{54.95}{24.02}$ & $\mathbf{\acc{92.35}{4.02}}$ & $\acc{93.75}{3.89}$
%   & $\acc{61.29}{6.02}$ & $\mathbf{\acc{61.88}{6.15}}$ & $\mathbf{\acc{64.47}{6.74}}$ \\
% \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4.5pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{PFL accuracy comparison over clients from a single seed.
% $\mathrm{acc}^{t}$ is the accuracy after $t$ local fine-tuning steps, reported
% as mean$_{\pm\text{std}}$; $\mathrm{acc}^{0}$ is given as the mean only.
% Multi CL requires known groups and is not deployable on real annotators
% (``--''). \textbf{Bold} marks the best value in each post-adaptation column.}
% \label{tab:pfl}
% \vspace{-8pt}
% \begin{tabular}{l ccc ccc ccc}
% \toprule
% & \multicolumn{3}{c}{Balanced (Synthetic)}
% & \multicolumn{3}{c}{Imbalanced (Synthetic)}
% & \multicolumn{3}{c}{Real-world} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% Algorithm & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{10}$ & $\mathrm{acc}^{80}$
%           & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{10}$ & $\mathrm{acc}^{80}$
%           & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{80}$ & $\mathrm{acc}^{240}$ \\
% \midrule
% Local
%   & 49.20 & $\acc{49.95}{7.26}$ & $\acc{58.05}{7.69}$
%   & 50.25 & $\acc{51.30}{7.44}$ & $\acc{58.70}{7.07}$
%   & 51.24 & $\acc{52.12}{6.65}$ & $\acc{54.59}{7.66}$ \\
% \midrule
% CL
%   & 51.80 & $\acc{53.70}{7.15}$ & $\acc{55.40}{5.99}$
%   & 56.00 & $\acc{56.90}{10.89}$ & $\acc{62.60}{7.93}$
%   & 58.06 & $\acc{57.06}{9.08}$ & $\acc{61.00}{6.69}$ \\
% Multi CL
%   & 92.10 & $\acc{92.15}{3.88}$ & $\acc{91.60}{4.29}$
%   & 92.30 & $\acc{91.70}{3.63}$ & $\acc{91.60}{3.67}$
%   & -- & -- & -- \\
% FL~\cite{mcmahan2017communication}
%   & 50.35 & $\acc{92.45}{3.76}$ & $\mathbf{\acc{94.70}{2.92}}$
%   & 55.60 & $\acc{90.55}{5.20}$ & $\mathbf{\acc{93.80}{3.40}}$
%   & 60.82 & $\acc{61.53}{7.70}$ & $\acc{63.00}{9.10}$ \\
% \midrule
% FedBiscuit~\cite{wu2024towards}
%   & 68.80 & $\acc{66.90}{6.18}$ & $\acc{71.45}{10.35}$
%   & 78.45 & $\acc{77.85}{9.85}$ & $\acc{80.80}{8.46}$
%   & 59.12 & $\acc{58.53}{6.76}$ & $\acc{57.06}{5.77}$ \\
% Soft-FL
%   & 51.70 & $\acc{62.40}{7.51}$ & $\acc{71.30}{6.09}$
%   & 56.50 & $\acc{75.95}{9.81}$ & $\acc{86.20}{7.41}$
%   & 60.88 & $\acc{58.71}{7.45}$ & $\acc{57.00}{9.07}$ \\
% \alg (ours)
%   & 49.15 & $\mathbf{\acc{94.55}{3.58}}$ & $\acc{94.30}{3.86}$
%   & 54.95 & $\mathbf{\acc{92.35}{4.02}}$ & $\acc{93.75}{3.89}$
%   & 60.59 & $\mathbf{\acc{61.71}{5.98}}$ & $\mathbf{\acc{64.41}{6.79}}$ \\
% \bottomrule
% \end{tabular}
% \end{table*}


\section{Experiments and Results}
\label{sec:exp}
We first evaluate the overall personalization performance of \alg\ on synthetic and real-world datasets. After we verify the proposed mechanism through the diagnostic metrics and examine the robustness of \alg\ with respect to the number of clusters $K$. Additional ablation studies and optimization sensitivity analyses are provided in Appendix~\ref{appsec:additional_results}.


% \smallskip
\noindent\textbf{Implementation Details.}\quad Unless explicitly mentioned, all experiments follow the configuration. We run 400 communication rounds of FL, sampling five clients per round ($|S_r| = 5$, $|G_r| = 5$ for our methods), and each selected client performs exactly 30 local training iterations per round with a batch size of 16, using AdamW~\cite{loshchilov2018decoupled} with $(\beta_1, \beta_2) = (0.9, 0.95)$ and a constant learning rate of $1\times10^{-5}$. In configurations with multiple global models and dynamic client--model assignment, the assignments are refreshed every $T=20$ rounds, and FedGD uses a mixing coefficient of $w=0.6$. Methods that maintain multiple server-side models use $K=4$ unless stated otherwise. Qwen2-0.5B~\cite{yang2024qwen2technicalreport} is used as the base model, and LoRA-based parameter-efficient tuning~\cite{hu2022lora, houlsby2019parameter} is applied with rank $r=8$, scaling factor $\alpha=16$, and dropout rate $0.05$. Following the standard Transformer architecture~\cite{vaswani2017attention}, LoRA is injected into the attention projection layers (\texttt{q\_proj}, \texttt{k\_proj}, \texttt{v\_proj}, \texttt{o\_proj}) and the MLP projection layers (\texttt{gate\_proj}, \texttt{up\_proj}) of all 24 Transformer blocks, yielding 24 LoRA-adapted layers over which we compute our layer-wise diagnostics. All experiments are implemented on top of the FedBiscuit~\cite{wu2024towards} codebase.

\noindent\textbf{Baselines.}\quad
Beyond CL, FL, and Multi-CL of Section~\ref{sec:motivation}, we compare three
deployable methods that do not assume known groups.
\begin{itemize}
\setlength\itemsep{2pt}
\item \textbf{Local:} fine-tunes the frozen backbone with LoRA on each client,
without a global phase.
\item \textbf{FedBiscuit}~\citep{wu2024towards}\textbf{:} maintains $K$ expert models on the server. At each communication round, every client receives its assigned expert model, performs local training, and uploads the updated model only to that expert for expert-specific aggregation. Every $T$ communication rounds, clients are reassigned to the expert with the lowest validation loss.
\item \textbf{Soft-FL:} replaces the hard client-to-expert assignment in FedBiscuit with validation-based soft weights over the $K$ experts. At each communication round, every client receives a weighted fusion of the $K$ expert models for local training, and the resulting local model contributes to every expert-specific aggregation according to the client's validation-based weights. See Appendix~\ref{appsec:alg_details} for details. 
\end{itemize}


% \begin{table}[ht]
% \centering
% \small
% \renewcommand{\arraystretch}{1.15}
% \caption{Real-world results across backbones, averaged over clients.
% $\mathrm{acc}^{t}$ is the accuracy after $t$ local fine-tuning steps, with
% $\mathrm{acc}^{0}$ in parentheses.}
% \label{tab:realworld}
% \vspace{-8pt}
% \begin{tabular*}{\columnwidth}{@{} l @{\hspace{6pt}\extracolsep{\fill}} cc @{}}
% \toprule
% Method & Qwen-1.5B & Gemma-2B \\
% \midrule
% Base & $\acc{61.12}{8.25}$ (49.59) & $\acc{67.71}{7.69}$ (58.53) \\
% CL   & $\acc{64.53}{7.44}$ (63.71) & $\acc{66.41}{7.14}$ (64.65) \\
% FL   & $\acc{68.53}{7.86}$ (67.88) & $\acc{71.47}{6.98}$ (71.29) \\
% FedGD (ours) & $\acc{0.00}{0.00}$ (0.00) & $\acc{0.00}{0.00}$ (0.00) \\
% \bottomrule
% \end{tabular*}
% \end{table}




\subsection{Main Results}

Table~\ref{tab:pfl} compares the deployable methods after 400 communication rounds. \alg attains the highest post-adaptation accuracy in every setting: $\mathrm{acc}^{10}=94.55$ under balanced groups, $92.35$ under imbalance, and $\mathrm{acc}^{240}=64.41$ in the real-world setting. \alg does so from the weakest starting point among all federated methods---$49.15$ and $54.95$ on the synthetic datasets, close to random guessing. The federated phase therefore learns an initialization optimized for rapid personalization rather than high pre-adaptation accuracy.



Group-specific initializations do not necessarily improve personalization and can even degrade real-world performance. Even with ground-truth preference groups, Multi-CL gains only marginally ($92.10\% \to 92.15\%$ at step 10) and eventually degrades ($91.60\%$ after 80 steps). Similarly, in the balanced synthetic setting, FedBiscuit achieves an accuracy of only $66.90\%$ after 10 adaptation steps, far behind standard FedAvg ($92.45\%$). On the real-world dataset, both FedBiscuit ($59.12\% \to 57.06\%$) and Soft-FL ($60.88\% \to 57.00\%$) experience performance degradation during personalization, ultimately finishing below single-model CL ($61.00\%$). These results demonstrate that learning separate initializations is ineffective when preference groups are unknown or imperfectly defined.


\begin{table}[t!]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\caption{Real-world results across different models. $\mathrm{acc}^{240}$ is
reported as mean$_{\pm\text{std}}$ over clients, marked with \textbf{Bold} for the best one, and $\mathrm{acc}^{0}$ as the mean before personalization.}
\label{tab:realworld}
\vspace{-8pt}
\begin{tabular*}{\columnwidth}{@{}l@{\extracolsep{\fill}}cccc@{}}
\toprule
& \multicolumn{2}{c}{Qwen-1.5B}
& \multicolumn{2}{c}{Gemma-2B} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
Method
& $\mathrm{acc}^{0}$
& $\mathrm{acc}^{240}$
& $\mathrm{acc}^{0}$
& $\mathrm{acc}^{240}$ \\
\midrule
Local
& 49.59
& $\acc{61.12}{8.25}$
& 58.53
& $\acc{67.71}{7.69}$ \\

CL
& 63.71
& $\acc{64.53}{7.44}$
& 64.65
& $\acc{66.41}{7.14}$ \\

FL
& 67.88
& $\acc{68.53}{7.86}$
& 71.29
& $\acc{71.47}{6.98}$ \\

\alg\ (ours)
& 68.65
& $\mathbf{\acc{70.29}{8.35}}$
& 70.29
& $\mathbf{\acc{72.35}{7.44}}$ \\
\bottomrule
\end{tabular*}
\end{table}



% \begin{table*}[t]
% \centering
% \caption{Effect of the number of clusters $K$ on FedGD under the imbalanced
% setting. $GQ(l)$ is the mean$\pm$std over the 24 layers, with its Body and Head
% averages. At $\theta_0$, $m^{0}$ and $H^{0}$ are the mean margin and headroom over
% each set, and $\Delta m^{10}$ the margin change after 10 steps. Accuracy is given
% with the initial accuracy in parentheses.}
% \label{tab:kdiag}
% \setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l ccc cc cc cccc cc c}
% \toprule
% & \multicolumn{3}{c}{Flatness ($\downarrow$)}
% & \multicolumn{2}{c}{Retention ($\mathcal{R}$, \%, $\uparrow$)}
% & \multicolumn{2}{c}{Correction ($\mathcal{W}$, \%, $\uparrow$)}
% & \multicolumn{4}{c}{Init.\ margin \& headroom ($\theta_0$)}
% & \multicolumn{2}{c}{$\Delta m^{10}$}
% & \multicolumn{1}{c}{Accuracy (\%, $\uparrow$)} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12} \cmidrule(lr){13-14} \cmidrule(lr){15-15}
% method & $GQ(l)$ & $GQ_{\mathcal{B}}$ & $GQ_{\mathcal{H}}$
%        & $H^{+}_{\mathcal{R}}$ & $P^{10}_{\mathcal{R}}$
%        & $H^{+}_{\mathcal{W}}$ & $P^{10}_{\mathcal{W}}$
%        & $m^{0}_{\mathcal{R}}$ & $m^{0}_{\mathcal{W}}$ & $H^{0}_{\mathcal{R}}$ & $H^{0}_{\mathcal{W}}$
%        & $\Delta m^{10}_{\mathcal{R}}$ & $\Delta m^{10}_{\mathcal{W}}$
%        & $\mathrm{acc}^{10}\,(\mathrm{acc}^{0})$ \\
% \midrule
% \alg ($K=2$)
%   & $0.18 \pm 0.02$ & 0.19 & 0.16 & 65.10 & 94.70 & 94.03 & 85.42
%   & $+3.76$ & $-2.94$ & 0.01 & 0.14 & $+1.35$ & $+6.41$ & 91.00 (60.90) \\
% \alg ($K=3$)
%   & $0.29 \pm 0.03$ & 0.31 & 0.26 & 69.72 & 95.20 & 90.76 & 89.72
%   & $+4.23$ & $-4.18$ & 0.10 & 0.32 & $+2.16$ & $+10.02$ & 92.80 (55.80) \\
% \alg ($K=4$)
%   & $0.27 \pm 0.02$ & 0.28 & 0.24 & 75.78 & 93.42 & 93.44 & 90.62
%   & $+3.59$ & $-3.65$ & 0.11 & 0.40 & $+2.59$ & $+8.94$ & 92.35 (54.95) \\
% % FedGD ($K=5$)
% %   & $0.55 \pm 0.03$ & 0.57 & 0.53 & 74.65 & 94.40 & 92.19 & 87.40
% %   & $+7.03$ & $-6.12$ & 0.77 & 1.94 & $+5.19$ & $+15.19$ & 91.60 (60.20) \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


\begin{table*}[t]
\centering
\caption{Effect of the number of clusters $K$ on \alg\ under the imbalanced
setting. $GQ(l)$ is the mean$\pm$std over the 24 LoRA layers. $m^{0}$ denotes
the mean reward margin at $\theta_{0}$. $P^{10}$ is the fraction of samples
correctly classified after 10 local steps. Accuracy is reported with the
initial accuracy in parentheses.}
\label{tab:kdiag}
\setlength{\tabcolsep}{3pt}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l ccc cc c c c}
\toprule
& \multicolumn{3}{c}{Flatness ($\downarrow$)}
& \multicolumn{2}{c}{Init.\ margin ($\theta_0$)}
& \multicolumn{1}{c}{Retention (\%, $\uparrow$)}
& \multicolumn{1}{c}{Correction (\%, $\uparrow$)}
& Accuracy (\%, $\uparrow$) \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){9-9}
Method
& $GQ(l)$ & $GQ_{\mathcal{B}}$ & $GQ_{\mathcal{H}}$
& $m_{\mathcal{R}}^{0}$ & $m_{\mathcal{W}}^{0}$
& $P_{\mathcal{R}}^{10}$
& $P_{\mathcal{W}}^{10}$
& $\mathrm{acc}^{10}\,(\mathrm{acc}^{0})$ \\
\midrule
\alg\ ($K=2$)
& $0.18 \pm 0.02$ & 0.19 & 0.16
& $+3.76$ & $-2.94$
& 94.70
& 85.42
& 91.00 (60.90) \\

\alg\ ($K=3$)
& $0.29 \pm 0.03$ & 0.31 & 0.26
& $+4.23$ & $-4.18$
& 95.20
& 89.72
& 92.80 (55.80) \\

\alg\ ($K=4$)
& $0.27 \pm 0.02$ & 0.28 & 0.24
& $+3.59$ & $-3.65$
& 93.42
& 90.62
& 92.35 (54.95) \\
\bottomrule
\end{tabular}
}
\end{table*}





Longer federated training substantially reduces the effect of group imbalance. Under the 200-round budget of Section~\ref{sec:motivation}, FL reaches only $\mathrm{acc}^{10}=61.75$ under the imbalanced setting (Table~\ref{tab:imbalanced}), whereas extending training to 400 rounds improves it to $90.55$, indicating that group imbalance slows rather than prevents federated optimization. Nevertheless, \alg still achieves the highest accuracy after only $R/2=200$ rounds of federated training. On the synthetic datasets, FL eventually catches up after sufficient personalization ($93.75$ vs.\ $93.80$ under imbalance and $94.30$ vs.\ $94.70$ under balanced groups), indicating that the benefit of the debiased initialization lies in faster adaptation rather than a better final optimum. 


\alg outperforms the baselines across larger models (Table~\ref{tab:realworld}).
On both Qwen 1.5B~\cite{yang2024qwen2technicalreport} and Gemma-2B~\cite{gemmateam2024gemmaopenmodelsbased}, \alg achieves the best
post-adaptation accuracy, and the gain comes from personalization rather than
from a stronger starting point. On Gemma-2B, \alg improves from $70.29$ to
$72.35$ while starting below FL, which gains only $0.18$ points
($71.29 \rightarrow 71.47$). On Qwen-1.5B, \alg improves by $1.64$ points
against FL's $0.65$.



% \begin{table*}[ht]
% \centering
% \small
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{Effect of $K$ on personalized accuracy, as mean$_{\pm\text{std}}$ over
% clients. FedGD is best at every $K$ (highlighted) and varies little across it,
% unlike the clustered baselines.}
% \label{tab:cluster}
% \vspace{-8pt}
% \begin{tabular}{l cccc cccc}
% \toprule
% & \multicolumn{4}{c}{Synthetic Imbalance ($\mathrm{acc}^{80}$)}
% & \multicolumn{4}{c}{Real-world ($\mathrm{acc}^{240}$)} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% Method & $K{=}2$ & $K{=}3$ & $K{=}4$ & $K{=}5$
%        & $K{=}2$ & $K{=}3$ & $K{=}4$ & $K{=}5$ \\
% \midrule
% FedBiscuit
%   & $\acc{73.50}{13.53}$ & $\acc{76.95}{12.16}$ & $\acc{80.80}{8.46}$ & $\acc{79.70}{9.43}$
%   & $\acc{58.94}{6.29}$ & $\acc{57.52}{7.50}$ & $\acc{57.06}{5.77}$ & $\acc{57.24}{6.88}$ \\
% Soft-FL
%   & $\acc{84.45}{6.35}$ & $\acc{86.30}{6.16}$ & $\acc{86.20}{7.41}$ & $\acc{87.50}{6.01}$
%   & $\acc{57.23}{8.30}$ & $\acc{56.77}{8.56}$ & $\acc{57.00}{9.07}$ & $\acc{59.00}{7.58}$ \\
% \rowcolor{fthl}
% FedGD (ours)
%   & $\acc{93.50}{3.73}$ & $\acc{93.65}{3.54}$ & $\acc{93.75}{3.89}$ & $\acc{93.15}{4.02}$
%   & $\acc{62.24}{6.94}$ & $\acc{62.24}{6.94}$ & $\acc{63.06}{8.18}$ & $\acc{64.47}{6.74}$ \\
% \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table}[t]
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{1.0}
% \caption{Effect of the number of clusters $K$ on personalized accuracy,
% averaged over clients.}
% \label{tab:cluster}
% \vspace{-8pt}
% \begin{tabular*}{\columnwidth}{@{} l @{\hspace{8pt}\extracolsep{\fill}} cccc @{\hspace{10pt}\extracolsep{\fill}} cccc @{}}
% \toprule
% & \multicolumn{4}{c}{Imbalanced ($\mathrm{acc}^{80}$)}
% & \multicolumn{4}{c}{Real-world ($\mathrm{acc}^{240}$)} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% Method & $2$ & $3$ & $4$ & $5$ & $2$ & $3$ & $4$ & $5$ \\
% \midrule
% FedBiscuit   & 73.50 & 76.95 & 80.80 & 79.70 & 58.94 & 57.52 & 57.06 & 57.24 \\
% Soft-FL      & 84.45 & 86.30 & 86.20 & 87.50 & 57.23 & 56.77 & 57.00 & 59.00 \\
% FedGD (ours) & 93.50 & 93.65 & 93.75 & 93.15 & 62.24 & 62.24 & 63.06 & 64.47 \\
% \bottomrule
% \end{tabular*}
% \end{table}



\subsection{Robustness to the Choice of $K$}

\alg does not require identifying the true preference groups.
Section~\ref{sec:motivation} showed that the degradation under imbalance
originates from biased client sampling rather than an incorrect partition.
Accordingly, \alg only requires a partition that removes the sampling
bias, rather than exactly recovering the preference groups.

Figure~\ref{fig:clusters} illustrates this mechanism. With ground-truth
groups G1 (Elementary \& Humorous), G2 (Elementary \& Non-Humorous),
G3 (PhD \& Humorous), and G4 (PhD \& Non-Humorous), \alg forms the
partitions $\{G1,G2\}$ and $\{G3,G4\}$ for $K=2$, preserving the shared
education attribute while balancing the humor attribute within each
partition. Increasing $K$ to three further separates G1 and G2, resulting
in the partitions $\{G1\}$, $\{G2\}$, and $\{G3,G4\}$. This preserves both
education and humor information for the Elementary clients, while the
PhD partition continues to average over the humor attribute. Only $K=4$
produces the partitions $\{G1\}$, $\{G2\}$, $\{G3\}$, and $\{G4\}$,
preserving both attributes for every group.

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{fig/fedgd_cluster_strip.pdf}
    \caption{Phase~1 clustering results under the synthetic imbalance setting for different numbers of experts ($K$). Clients are colored by their assigned expert (lowest validation loss).}
    \label{fig:clusters}
\end{figure}

Despite these different partitions, Table~\ref{tab:kdiag} demonstrates that the results retain robust optimization. Across all three values of $K$, the learned models maintain low curvature ($GQ(l)\le0.29$), remain near the decision boundary with narrow initial margins, and achieve high correction rates just 10 local steps. As a result, the accuracy varies marginally, within a range of $91.0\%$ to $ 92.8\%$.

These results indicate that recovering the exact preference groups is
not necessary. Once the discovered partition sufficiently removes the biased client sampling, the resulting initialization retains the flatness and under-confident margins enabling rapid local adaptation, making \alg
largely insensitive to the choice of $K$.


% Section~\ref{sec:motivation} demonstrated that performance degradation under group imbalance is due to biased client sampling rather than incorrect partitioning. Consequently, FedGD does not require $K$ to match the true number of preference groups, as long as the partition adequately mitigates sampling bias. As shown in Table~\ref{tab:kdiag}, even when $K=2$ merges multiple preference groups, FedGD still learns balanced representations ($GQ(l)=0.18$), initializes near the decision boundary ($m_{\mathcal W}^{0}=+3.76$), and achieves $91.00\%$ post-adaptation accuracy. While larger $K$ slightly refines the partition, performance remains within $1.35\%$ across all choices after 10 personalization steps, confirming that exact group recovery is not required.


% FedGD does not require $K$ to match the true number of preference groups. Section~\ref{sec:motivation} showed that the failure under imbalance originates from biased client sampling rather than an incorrect partition: FL\_target changes only the sampling distribution and recovers the behavior of FL under balanced groups. A partition therefore needs only to remove the sampling bias, rather than exactly recover the underlying preference groups.

% Table~\ref{tab:kdiag} shows that this remains true even when $K$ is smaller than the true number of preference groups. With $K=2$, multiple preference groups are merged into the same cluster, yet FedGD still learns similarly flat representations ($GQ(l)=0.18$), initializes close to the decision boundary ($m_{\mathcal W}^{0}=+3.76$), and achieves $91.00\%$ post-adaptation accuracy. Increasing $K$ to three or four further refines the partition and slightly improves performance, but all three choices of $K$ remain within $1.35$ points after ten personalization steps.

% These results confirm that exact group recovery is sufficient but not necessary. FedGD does not require recovering every latent preference group; it requires only a partition that sufficiently removes the sampling bias.




==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/06_related.tex <==
\section{Related Work}
\label{sec:related}


\noindent\textbf{Reward modeling under preference heterogeneity.}\quad
Reward models trained on preference data are central to alignment pipelines \citep{stiennon2020learning, ouyang2022training}, alongside alternatives such as DPO~\citep{rafailov2023direct} and RRHF~\citep{yuan2023rrhf}. To accommodate diverse users, recent methods absorb the variation into the structure of one centralized model, including group-wise robust objectives~\citep{ramesh2024group}, multi-objective reward heads~\citep{wang2024arithmetic}, routing over latent subgroups~\citep{shen2025micro}, latent user variables~\citep{poddar2024personalizing}, and post-hoc merging of objective-specific policies~\citep{jang2023personalized}, so that a single deployed model can be steered per user. All of these approaches assume centralized access to preference data, which privacy regulation often precludes~\citep{regulation2016regulation, illman2019california, kopf2023openassistant}. Federated preference alignment removes this assumption by aggregating locally computed alignment updates~\citep{ye2024openfedllm, wu2024towards, fan2024fedrlhf}, but returning a single consensus policy limits its ability to serve heterogeneous clients, underscoring the need to leverage federated learning for local personalization.


\noindent\textbf{Multiple global models under heterogeneity.}\quad
When clients disagree in preference signals, a common method is to train multiple global models, one per group of similar clients. FedBiscuit~\citep{wu2024towards} clusters clients by preference similarity and trains one reward model per cluster, the design our experiments compare against. FedLEASE~\citep{wang2025adaptive}, IFCA~\citep{ghosh2020efficient}, CFL~\citep{sattler2020clustered}, and FeSEM~\citep{long2023multi} likewise partition clients by preference or domain similarity, while soft membership~\citep{ruan2022fedsoft} and mixture-of-experts approaches~\citep{yi2024pfedmoe} offer more flexible combinations. These designs rest on the premise that a client is better served by a model that never averaged over conflicting objectives. A complementary line of personalized federated learning instead keeps one global model. It defers personalization to local adaptation, either by training the global model as an initialization for a few local gradient steps~\citep{fallah2020personalized, dinh2020personalized, oh2021fedbabu} or by sharing a common representation while keeping heads or lightweight adapters client-specific~\citep{collins2021exploiting, li2021ditto, yi2023pfedlora, scott2024pefll}, and biased client participation in this setting can be corrected through clustered or importance-based sampling~\citep{fraboni2021clustered, chen2022optimal}. However, prior work evaluates models primarily at the global level, so a deeper analysis is needed to examine performance trends after local fine-tuning, thereby clarifying the true role of client grouping.



==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/sec/07_conclusion.tex <==
\vspace{-7pt}
\section{Conclusion}
\label{sec:conclusion}
We examined what constitutes a good initialization for personalized reward modeling under conflicting preferences. The prevailing response to such conflict is to partition clients and train one model per group, on the premise that a client is better served by a model that never averaged over opposing labels. Our results do not support this premise. A single federated model performs at chance before adaptation, yet a few local steps carry it past a centralized model trained on the client's own ground-truth group. Averaging cancels the opposing label choices while retaining the distinction clients agree on, leaving the initialization in a flat region from which successive local steps remain aligned. When the preference groups differ in size the cancellation becomes asymmetric: the shared model commits to the majority side and leaves minority clients too far from the decision boundary for a few local steps to recover. \alg restores the symmetry by discovering the groups during federated training and debiasing the client sampling over them.












==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/tables/gfl_acc_all.tex <==
% \begin{table*}[t!]
%     \centering
%     \small
%     \vspace{-2pt}
%     \caption{Accuracy comparison in the GFL setting. 
%     %We used MobileNet and checked CIFAR-10/100 datasets under sharding/LDA non-iidness settings. 
%     The entries are based on results obtained from three different seeds, indicating the mean and standard deviation of the accuracy of the global model, represented as X{\tiny $\pm$Y}. The best performance in each case is highlighted in \textbf{bold}.}
%     \label{tab:gfl_acc_all}
%     \vspace{-14pt}
%     \resizebox{.64\textwidth}{!}{
%     \begin{tabular}{l|cccc|ccc}
%       \toprule 
%       \multicolumn{8}{c}{\textbf{NIID Partition Strategy: Sharding}}\\ \midrule
%        & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c}{VGG on CIFAR-10}\\  \cmidrule{2-8}
%       Algorithm & $s$=10 & $s$=20 & $s$=50 & $s$=100  & $s$=2 & $s$=5 & $s$=10\\ \midrule
%       FedAvg~\cite{mcmahan2017communication}  & 36.63{\tiny $\pm$ 0.22} & 42.25{\tiny $\pm$ 1.42} & 45.57{\tiny $\pm$ 0.22} & 48.20{\tiny $\pm$ 1.36} & 72.08{\tiny $\pm$ 0.67} & 81.53{\tiny $\pm$ 0.35} & 82.38{\tiny $\pm$ 0.40}   \\ 

%       SCAFFOLD~\cite{karimireddy2020scaffold}\,($\times 2$)\!\!
%       & 46.08{\tiny $\pm$ 0.37} & 48.15{\tiny $\pm$ 1.21} & 49.31{\tiny $\pm$ 0.62} & 50.73{\tiny $\pm$ 0.42} & 75.49{\tiny $\pm$ 0.42} & \textbf{84.14}{\tiny $\pm$ 0.13} & \textbf{85.11}{\tiny $\pm$ 0.29}   \\ 

%       FedNTD~\cite{lee2022preservation}  & 34.05{\tiny $\pm$ 1.19} & 41.78{\tiny $\pm$ 0.31} & 46.42{\tiny $\pm$ 0.63} & 47.17{\tiny $\pm$ 0.32} & 72.21{\tiny $\pm$ 0.59} & 69.96{\tiny $\pm$ 17.10} & 81.99{\tiny $\pm$ 0.42}   \\ 
%       FedExP~\cite{jhunjhunwala2023fedexp}  & 36.85{\tiny $\pm$ 0.11} & 42.49{\tiny $\pm$ 1.22} & 45.07{\tiny $\pm$ 0.92} & 48.09{\tiny $\pm$ 1.00} & 72.31{\tiny $\pm$ 0.60} & 81.41{\tiny $\pm$ 0.19} & 82.47{\tiny $\pm$ 0.16}   \\ \midrule

%       FedBABU~\cite{oh2021fedbabu}  & 45.97{\tiny $\pm$ 0.48} & 45.53{\tiny $\pm$ 0.79} & 46.52{\tiny $\pm$ 0.51} & 46.02{\tiny $\pm$ 0.28} & 71.99{\tiny $\pm$ 0.52} & 81.07{\tiny $\pm$ 0.60} & 82.32{\tiny $\pm$ 0.06}   \\ 
      
%       SphereFed~\cite{dong2022spherefed} & 42.71{\tiny $\pm$ 0.65} & 48.63{\tiny $\pm$ 0.90} & {\textbf{52.16}}{\tiny $\pm$ 0.22} & \textbf{53.41}{\tiny $\pm$ 0.19} & \textbf{76.33}{\tiny $\pm$ 0.33} & 83.67{\tiny $\pm$ 0.18} & 84.36{\tiny $\pm$ 0.30}   \\ 
%       FedETF~\cite{li2023no} & 31.37{\tiny $\pm$ 0.72} & 42.22{\tiny $\pm$ 0.77} & 47.47{\tiny $\pm$ 0.67} & 49.00{\tiny $\pm$ 0.74} & 67.81{\tiny $\pm$ 0.94} & 80.78{\tiny $\pm$ 0.68} & 82.60{\tiny $\pm$ 0.46}   \\ 
%       \alg \textbf{(Ours)} & \textbf{48.21}{\tiny $\pm$ 0.56} & \textbf{50.77}{\tiny $\pm$ 0.14} & {\textbf{52.15}}{\tiny $\pm$ 0.03} & \textbf{52.41}{\tiny $\pm$ 0.81} & \textbf{76.57}{\tiny $\pm$ 0.51} & 83.22{\tiny $\pm$ 0.34} & 84.14{\tiny $\pm$ 0.27}   \\ \bottomrule
%       \midrule
%       \multicolumn{8}{c}{\textbf{NIID Partition Strategy: LDA}}\\ \midrule
%         & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c}{VGG on CIFAR-10} \\  \cmidrule{2-8}
%       Algorithm & $\alpha$=0.05 & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3  & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3\\ \midrule
%       FedAvg~\cite{mcmahan2017communication}  & 35.58{\tiny $\pm$ 1.35} & 42.10{\tiny $\pm$ 0.60} & 44.78{\tiny $\pm$ 0.72} & 45.73{\tiny $\pm$ 0.88} & 68.71{\tiny $\pm$ 1.82} & 77.75{\tiny $\pm$ 0.26} & 80.76{\tiny $\pm$ 0.51}   \\ 

%       SCAFFOLD~\cite{karimireddy2020scaffold}\,($\times 2$)\!\! & 40.54{\tiny $\pm$ 0.48} & 46.14{\tiny $\pm$ 0.70} & 47.98{\tiny $\pm$ 0.93} & 48.06{\tiny $\pm$ 1.08} & \textit{(Failed)} & 80.15{\tiny $\pm$ 0.29} & {\textbf{82.63}}{\tiny $\pm$ 0.23}   \\ 

%       FedNTD~\cite{lee2022preservation}  & 31.78{\tiny $\pm$ 3.14} & 40.41{\tiny $\pm$ 0.96} & 43.10{\tiny $\pm$ 2.03} & 43.04{\tiny $\pm$ 0.82} & 70.22{\tiny $\pm$ 0.40} & 77.16{\tiny $\pm$ 0.20} & 79.50{\tiny $\pm$ 0.56}   \\ 
%       FedExP~\cite{jhunjhunwala2023fedexp}  & 34.39{\tiny $\pm$ 1.77} & 40.85{\tiny $\pm$ 1.32} & 44.47{\tiny $\pm$ 0.28} & 45.44{\tiny $\pm$ 0.14} & 70.14{\tiny $\pm$ 0.53} & 78.09{\tiny $\pm$ 0.21} & 80.40{\tiny $\pm$ 0.54}   \\ \midrule

%       FedBABU~\cite{oh2021fedbabu}  & 41.97{\tiny $\pm$ 1.01} & 45.77{\tiny $\pm$ 0.28} & 44.28{\tiny $\pm$ 0.45} & 44.80{\tiny $\pm$ 0.63} & 65.15{\tiny $\pm$ 3.66} & 77.03{\tiny $\pm$ 0.25} & 79.91{\tiny $\pm$ 0.13}   \\ 
      
%       SphereFed~\cite{dong2022spherefed} & 39.56{\tiny $\pm$ 0.48} & 46.54{\tiny $\pm$ 0.58} & \textbf{49.41}{\tiny $\pm$ 0.78} & 49.22{\tiny $\pm$ 0.86} & 67.49{\tiny $\pm$ 3.49} & 80.05{\tiny $\pm$ 0.40} & {\textbf{82.62}}{\tiny $\pm$ 0.66}   \\ 
%       FedETF~\cite{li2023no} & 40.71{\tiny $\pm$ 0.90} & 45.63{\tiny $\pm$ 0.33} & 46.28{\tiny $\pm$ 1.05} & 46.69{\tiny $\pm$ 0.87} & 70.75{\tiny $\pm$ 0.36} & 77.86{\tiny $\pm$ 0.46} & 79.95{\tiny $\pm$ 0.34}   \\ 
%       \alg \textbf{(Ours)} & \textbf{45.12}{\tiny $\pm$ 1.00} & \textbf{49.48}{\tiny $\pm$ 0.50} & \textbf{50.67}{\tiny $\pm$ 0.88} & \textbf{51.15}{\tiny $\pm$ 0.65} & \textbf{72.07}{\tiny $\pm$ 2.26} & \textbf{80.90}{\tiny $\pm$ 0.02} & {\textbf{82.42}}{\tiny $\pm$ 0.10}   \\ \midrule
%     \end{tabular}
%     }
%     % \vspace{-10pt}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \small
%     \vspace{-2pt}
%     \caption{Accuracy comparison in the GFL setting. 
%     %We used MobileNet and checked CIFAR-10/100 datasets under sharding/LDA non-iidness settings. 
%     The entries are based on results obtained from three different seeds, indicating the mean and standard deviation of the accuracy of the global model, represented as X{\tiny $\pm$Y}. The best performance in each case is highlighted in \textbf{bold}.}
%     \label{tab:gfl_acc_all}
%     \vspace{-10pt}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|cccc|ccc|cccc|ccc}
%       \toprule 
%       \multicolumn{8}{c|}{\textbf{NIID Partition Strategy: Sharding}} & \multicolumn{7}{c}{\textbf{NIID Partition Strategy: LDA}}\\ \midrule
%        & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c|}{VGG on CIFAR-10} & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c}{VGG on CIFAR-10}\\  \cmidrule{2-15}
%       Algorithm & $s$=10 & $s$=20 & $s$=50 & $s$=100  & $s$=2 & $s$=5 & $s$=10 & $\alpha$=0.05 & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3  & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3\\ \midrule
%       FedAvg~\cite{mcmahan2017communication}  & 36.63{\tiny $\pm$ 0.22} & 42.25{\tiny $\pm$ 1.42} & 45.57{\tiny $\pm$ 0.22} & 48.20{\tiny $\pm$ 1.36} & 72.08{\tiny $\pm$ 0.67} & 81.53{\tiny $\pm$ 0.35} & 82.38{\tiny $\pm$ 0.40} & 35.58{\tiny $\pm$ 1.35} & 42.10{\tiny $\pm$ 0.60} & 44.78{\tiny $\pm$ 0.72} & 45.73{\tiny $\pm$ 0.88} & 68.71{\tiny $\pm$ 1.82} & 77.75{\tiny $\pm$ 0.26} & 80.76{\tiny $\pm$ 0.51}  \\ 

%       SCAFFOLD~\cite{karimireddy2020scaffold}\,($\times 2$)\!\!
%       & 46.08{\tiny $\pm$ 0.37} & 48.15{\tiny $\pm$ 1.21} & 49.31{\tiny $\pm$ 0.62} & 50.73{\tiny $\pm$ 0.42} & 75.49{\tiny $\pm$ 0.42} & \textbf{84.14}{\tiny $\pm$ 0.13} & \textbf{85.11}{\tiny $\pm$ 0.29} & 40.54{\tiny $\pm$ 0.48} & 46.14{\tiny $\pm$ 0.70} & 47.98{\tiny $\pm$ 0.93} & 48.06{\tiny $\pm$ 1.08} & \textit{(Failed)} & 80.15{\tiny $\pm$ 0.29} & {\textbf{82.63}}{\tiny $\pm$ 0.23} \\ 

%       FedNTD~\cite{lee2022preservation}  & 34.05{\tiny $\pm$ 1.19} & 41.78{\tiny $\pm$ 0.31} & 46.42{\tiny $\pm$ 0.63} & 47.17{\tiny $\pm$ 0.32} & 72.21{\tiny $\pm$ 0.59} & 69.96{\tiny $\pm$ 17.10} & 81.99{\tiny $\pm$ 0.42} & 31.78{\tiny $\pm$ 3.14} & 40.41{\tiny $\pm$ 0.96} & 43.10{\tiny $\pm$ 2.03} & 43.04{\tiny $\pm$ 0.82} & 70.22{\tiny $\pm$ 0.40} & 77.16{\tiny $\pm$ 0.20} & 79.50{\tiny $\pm$ 0.56} \\ 
%       FedExP~\cite{jhunjhunwala2023fedexp}  & 36.85{\tiny $\pm$ 0.11} & 42.49{\tiny $\pm$ 1.22} & 45.07{\tiny $\pm$ 0.92} & 48.09{\tiny $\pm$ 1.00} & 72.31{\tiny $\pm$ 0.60} & 81.41{\tiny $\pm$ 0.19} & 82.47{\tiny $\pm$ 0.16} & 34.39{\tiny $\pm$ 1.77} & 40.85{\tiny $\pm$ 1.32} & 44.47{\tiny $\pm$ 0.28} & 45.44{\tiny $\pm$ 0.14} & 70.14{\tiny $\pm$ 0.53} & 78.09{\tiny $\pm$ 0.21} & 80.40{\tiny $\pm$ 0.54} \\ \midrule

%       FedBABU~\cite{oh2021fedbabu}  & 45.97{\tiny $\pm$ 0.48} & 45.53{\tiny $\pm$ 0.79} & 46.52{\tiny $\pm$ 0.51} & 46.02{\tiny $\pm$ 0.28} & 71.99{\tiny $\pm$ 0.52} & 81.07{\tiny $\pm$ 0.60} & 82.32{\tiny $\pm$ 0.06} & 41.97{\tiny $\pm$ 1.01} & 45.77{\tiny $\pm$ 0.28} & 44.28{\tiny $\pm$ 0.45} & 44.80{\tiny $\pm$ 0.63} & 65.15{\tiny $\pm$ 3.66} & 77.03{\tiny $\pm$ 0.25} & 79.91{\tiny $\pm$ 0.13} \\ 
      
%       SphereFed~\cite{dong2022spherefed} & 42.71{\tiny $\pm$ 0.65} & 48.63{\tiny $\pm$ 0.90} & {\textbf{52.16}}{\tiny $\pm$ 0.22} & \textbf{53.41}{\tiny $\pm$ 0.19} & \textbf{76.33}{\tiny $\pm$ 0.33} & 83.67{\tiny $\pm$ 0.18} & 84.36{\tiny $\pm$ 0.30} & 39.56{\tiny $\pm$ 0.48} & 46.54{\tiny $\pm$ 0.58} & \textbf{49.41}{\tiny $\pm$ 0.78} & 49.22{\tiny $\pm$ 0.86} & 67.49{\tiny $\pm$ 3.49} & 80.05{\tiny $\pm$ 0.40} & {\textbf{82.62}}{\tiny $\pm$ 0.66} \\ 
%       FedETF~\cite{li2023no} & 31.37{\tiny $\pm$ 0.72} & 42.22{\tiny $\pm$ 0.77} & 47.47{\tiny $\pm$ 0.67} & 49.00{\tiny $\pm$ 0.74} & 67.81{\tiny $\pm$ 0.94} & 80.78{\tiny $\pm$ 0.68} & 82.60{\tiny $\pm$ 0.46} & 40.71{\tiny $\pm$ 0.90} & 45.63{\tiny $\pm$ 0.33} & 46.28{\tiny $\pm$ 1.05} & 46.69{\tiny $\pm$ 0.87} & 70.75{\tiny $\pm$ 0.36} & 77.86{\tiny $\pm$ 0.46} & 79.95{\tiny $\pm$ 0.34} \\ 
%       \alg \textbf{(Ours)} & \textbf{48.21}{\tiny $\pm$ 0.56} & \textbf{50.77}{\tiny $\pm$ 0.14} & {\textbf{52.15}}{\tiny $\pm$ 0.03} & \textbf{52.41}{\tiny $\pm$ 0.81} & \textbf{76.57}{\tiny $\pm$ 0.51} & 83.22{\tiny $\pm$ 0.34} & 84.14{\tiny $\pm$ 0.27} & \textbf{45.12}{\tiny $\pm$ 1.00} & \textbf{49.48}{\tiny $\pm$ 0.50} & \textbf{50.67}{\tiny $\pm$ 0.88} & \textbf{51.15}{\tiny $\pm$ 0.65} & \textbf{72.07}{\tiny $\pm$ 2.26} & \textbf{80.90}{\tiny $\pm$ 0.02} & {\textbf{82.42}}{\tiny $\pm$ 0.10} \\ \bottomrule
%     \end{tabular}
%     }
%     % \vspace{-10pt}
% \end{table*}


% \begin{table*}[t!]
%     \centering
%     \small
%     \vspace{-2pt}
%     \caption{Accuracy comparison in the GFL setting. The entries are based on results obtained from three different seeds, indicating the mean and standard deviation of the accuracy of the global model, represented as X{\tiny $\pm$Y}. The best performance in each case is highlighted in \textbf{bold}.}
%     \label{tab:gfl_acc_all}
%     \vspace{-10pt}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|cccc|ccc|cccc|ccc}
%       \toprule 
%       \multicolumn{8}{c|}{\textbf{NIID Partition Strategy: Sharding}} & \multicolumn{7}{c}{\textbf{NIID Partition Strategy: LDA}}\\ \midrule
%        & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c|}{VGG on CIFAR-10} & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c}{VGG on CIFAR-10}\\  \cmidrule{2-15}
%       Algorithm & $s$=10 & $s$=20 & $s$=50 & $s$=100  & $s$=2 & $s$=5 & $s$=10 & $\alpha$=0.05 & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3  & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3\\ \midrule
%       FedAvg~\cite{mcmahan2017communication}  & 36.63{\tiny $\pm$ 0.22} & 42.25{\tiny $\pm$ 1.42} & 45.57{\tiny $\pm$ 0.22} & 48.20{\tiny $\pm$ 1.36} & 72.08{\tiny $\pm$ 0.67} & 81.53{\tiny $\pm$ 0.35} & 82.38{\tiny $\pm$ 0.40} & 35.58{\tiny $\pm$ 1.35} & 42.10{\tiny $\pm$ 0.60} & 44.78{\tiny $\pm$ 0.72} & 45.73{\tiny $\pm$ 0.88} & 68.71{\tiny $\pm$ 1.82} & 77.75{\tiny $\pm$ 0.26} & 80.76{\tiny $\pm$ 0.51}  \\ 

%       SCAFFOLD~\cite{karimireddy2020scaffold}\,($\times 2$)\!\!
%       & 46.08{\tiny $\pm$ 0.37} & 48.15{\tiny $\pm$ 1.21} & 49.31{\tiny $\pm$ 0.62} & 50.73{\tiny $\pm$ 0.42} & 75.49{\tiny $\pm$ 0.42} & \textbf{\large 84.14}{\tiny $\pm$ 0.13} & \textbf{\large 85.11}{\tiny $\pm$ 0.29} & 40.54{\tiny $\pm$ 0.48} & 46.14{\tiny $\pm$ 0.70} & 47.98{\tiny $\pm$ 0.93} & 48.06{\tiny $\pm$ 1.08} & \textit{(Failed)} & 80.15{\tiny $\pm$ 0.29} & {\textbf{\large 82.63}}{\tiny $\pm$ 0.23} \\ 

%       FedNTD~\cite{lee2022preservation}  & 34.05{\tiny $\pm$ 1.19} & 41.78{\tiny $\pm$ 0.31} & 46.42{\tiny $\pm$ 0.63} & 47.17{\tiny $\pm$ 0.32} & 72.21{\tiny $\pm$ 0.59} & 69.96{\tiny $\pm$ 17.10} & 81.99{\tiny $\pm$ 0.42} & 31.78{\tiny $\pm$ 3.14} & 40.41{\tiny $\pm$ 0.96} & 43.10{\tiny $\pm$ 2.03} & 43.04{\tiny $\pm$ 0.82} & 70.22{\tiny $\pm$ 0.40} & 77.16{\tiny $\pm$ 0.20} & 79.50{\tiny $\pm$ 0.56} \\ 
%       FedExP~\cite{jhunjhunwala2023fedexp}  & 36.85{\tiny $\pm$ 0.11} & 42.49{\tiny $\pm$ 1.22} & 45.07{\tiny $\pm$ 0.92} & 48.09{\tiny $\pm$ 1.00} & 72.31{\tiny $\pm$ 0.60} & 81.41{\tiny $\pm$ 0.19} & 82.47{\tiny $\pm$ 0.16} & 34.39{\tiny $\pm$ 1.77} & 40.85{\tiny $\pm$ 1.32} & 44.47{\tiny $\pm$ 0.28} & 45.44{\tiny $\pm$ 0.14} & 70.14{\tiny $\pm$ 0.53} & 78.09{\tiny $\pm$ 0.21} & 80.40{\tiny $\pm$ 0.54} \\ \midrule

%       FedBABU~\cite{oh2021fedbabu}  & 45.97{\tiny $\pm$ 0.48} & 45.53{\tiny $\pm$ 0.79} & 46.52{\tiny $\pm$ 0.51} & 46.02{\tiny $\pm$ 0.28} & 71.99{\tiny $\pm$ 0.52} & 81.07{\tiny $\pm$ 0.60} & 82.32{\tiny $\pm$ 0.06} & 41.97{\tiny $\pm$ 1.01} & 45.77{\tiny $\pm$ 0.28} & 44.28{\tiny $\pm$ 0.45} & 44.80{\tiny $\pm$ 0.63} & 65.15{\tiny $\pm$ 3.66} & 77.03{\tiny $\pm$ 0.25} & 79.91{\tiny $\pm$ 0.13} \\ 
      
%       SphereFed~\cite{dong2022spherefed} & 42.71{\tiny $\pm$ 0.65} & 48.63{\tiny $\pm$ 0.90} & {\textbf{\large 52.16}}{\tiny $\pm$ 0.22} & \textbf{\large 53.41}{\tiny $\pm$ 0.19} & \textbf{\large 76.33}{\tiny $\pm$ 0.33} & 83.67{\tiny $\pm$ 0.18} & 84.36{\tiny $\pm$ 0.30} & 39.56{\tiny $\pm$ 0.48} & 46.54{\tiny $\pm$ 0.58} & \textbf{\large 49.41}{\tiny $\pm$ 0.78} & 49.22{\tiny $\pm$ 0.86} & 67.49{\tiny $\pm$ 3.49} & 80.05{\tiny $\pm$ 0.40} & {\textbf{\large 82.62}}{\tiny $\pm$ 0.66} \\ 
%       FedETF~\cite{li2023no} & 31.37{\tiny $\pm$ 0.72} & 42.22{\tiny $\pm$ 0.77} & 47.47{\tiny $\pm$ 0.67} & 49.00{\tiny $\pm$ 0.74} & 67.81{\tiny $\pm$ 0.94} & 80.78{\tiny $\pm$ 0.68} & 82.60{\tiny $\pm$ 0.46} & 40.71{\tiny $\pm$ 0.90} & 45.63{\tiny $\pm$ 0.33} & 46.28{\tiny $\pm$ 1.05} & 46.69{\tiny $\pm$ 0.87} & 70.75{\tiny $\pm$ 0.36} & 77.86{\tiny $\pm$ 0.46} & 79.95{\tiny $\pm$ 0.34} \\ 
%       \alg \textbf{(Ours)} & \textbf{\large 48.21}{\tiny $\pm$ 0.56} & \textbf{\large 50.77}{\tiny $\pm$ 0.14} & {\textbf{\large 52.15}}{\tiny $\pm$ 0.03} & \textbf{\large 52.41}{\tiny $\pm$ 0.81} & \textbf{\large 76.57}{\tiny $\pm$ 0.51} & 83.22{\tiny $\pm$ 0.34} & 84.14{\tiny $\pm$ 0.27} & \textbf{\large 45.12}{\tiny $\pm$ 1.00} & \textbf{\large 49.48}{\tiny $\pm$ 0.50} & \textbf{\large 50.67}{\tiny $\pm$ 0.88} & \textbf{\large 51.15}{\tiny $\pm$ 0.65} & \textbf{\large 72.07}{\tiny $\pm$ 2.26} & \textbf{\large 80.90}{\tiny $\pm$ 0.02} & {\textbf{\large 82.42}}{\tiny $\pm$ 0.10} \\ \bottomrule
%     \end{tabular}
%     }
%     % \vspace{-10pt}
% \end{table*}


\begin{table*}[t!]
    \centering
    \small
    \vspace{-2pt}
    \caption{Accuracy comparison in the GFL setting. The entries are based on results obtained from three different seeds, indicating the mean and standard deviation of the accuracy of the global model, represented as X{\tiny $\pm$Y}. The best performance in each case is highlighted in \mybold{bold}.}
    \label{tab:gfl_acc_all}
    \vspace{-10pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|ccc|cccc|ccc}
      \toprule 
      \multicolumn{8}{c|}{\mybold{NIID Partition Strategy: Sharding}} & \multicolumn{7}{c}{\mybold{NIID Partition Strategy: LDA}}\\ \midrule
       & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c|}{VGG on CIFAR-10} & \multicolumn{4}{c|}{MobileNet on CIFAR-100} & \multicolumn{3}{c}{VGG on CIFAR-10}\\  \cmidrule{2-15}
      Algorithm & $s$=10 & $s$=20 & $s$=50 & $s$=100  & $s$=2 & $s$=5 & $s$=10 & $\alpha$=0.05 & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3  & $\alpha$=0.1 & $\alpha$=0.2 & $\alpha$=0.3\\ \midrule
      FedAvg~\cite{mcmahan2017communication}  & 36.63{\tiny $\pm$ 0.22} & 42.25{\tiny $\pm$ 1.42} & 45.57{\tiny $\pm$ 0.22} & 48.20{\tiny $\pm$ 1.36} & 72.08{\tiny $\pm$ 0.67} & 81.53{\tiny $\pm$ 0.35} & 82.38{\tiny $\pm$ 0.40} & 35.58{\tiny $\pm$ 1.35} & 42.10{\tiny $\pm$ 0.60} & 44.78{\tiny $\pm$ 0.72} & 45.73{\tiny $\pm$ 0.88} & 68.71{\tiny $\pm$ 1.82} & 77.75{\tiny $\pm$ 0.26} & 80.76{\tiny $\pm$ 0.51}  \\ 

      SCAFFOLD~\cite{karimireddy2020scaffold}\,($\times 2$)\!\!
      & 46.08{\tiny $\pm$ 0.37} & 48.15{\tiny $\pm$ 1.21} & 49.31{\tiny $\pm$ 0.62} & 50.73{\tiny $\pm$ 0.42} & 75.49{\tiny $\pm$ 0.42} & \mybold{84.14}{\tiny $\pm$ 0.13} & \mybold{85.11}{\tiny $\pm$ 0.29} & 40.54{\tiny $\pm$ 0.48} & 46.14{\tiny $\pm$ 0.70} & 47.98{\tiny $\pm$ 0.93} & 48.06{\tiny $\pm$ 1.08} & \textit{(Failed)} & 80.15{\tiny $\pm$ 0.29} & {\mybold{82.63}}{\tiny $\pm$ 0.23} \\ 

      FedNTD~\cite{lee2022preservation}  & 34.05{\tiny $\pm$ 1.19} & 41.78{\tiny $\pm$ 0.31} & 46.42{\tiny $\pm$ 0.63} & 47.17{\tiny $\pm$ 0.32} & 72.21{\tiny $\pm$ 0.59} & 69.96{\tiny $\pm$ 17.10} & 81.99{\tiny $\pm$ 0.42} & 31.78{\tiny $\pm$ 3.14} & 40.41{\tiny $\pm$ 0.96} & 43.10{\tiny $\pm$ 2.03} & 43.04{\tiny $\pm$ 0.82} & 70.22{\tiny $\pm$ 0.40} & 77.16{\tiny $\pm$ 0.20} & 79.50{\tiny $\pm$ 0.56} \\ 
      FedExP~\cite{jhunjhunwala2023fedexp}  & 36.85{\tiny $\pm$ 0.11} & 42.49{\tiny $\pm$ 1.22} & 45.07{\tiny $\pm$ 0.92} & 48.09{\tiny $\pm$ 1.00} & 72.31{\tiny $\pm$ 0.60} & 81.41{\tiny $\pm$ 0.19} & 82.47{\tiny $\pm$ 0.16} & 34.39{\tiny $\pm$ 1.77} & 40.85{\tiny $\pm$ 1.32} & 44.47{\tiny $\pm$ 0.28} & 45.44{\tiny $\pm$ 0.14} & 70.14{\tiny $\pm$ 0.53} & 78.09{\tiny $\pm$ 0.21} & 80.40{\tiny $\pm$ 0.54} \\ \midrule

      FedBABU~\cite{oh2021fedbabu}  & 45.97{\tiny $\pm$ 0.48} & 45.53{\tiny $\pm$ 0.79} & 46.52{\tiny $\pm$ 0.51} & 46.02{\tiny $\pm$ 0.28} & 71.99{\tiny $\pm$ 0.52} & 81.07{\tiny $\pm$ 0.60} & 82.32{\tiny $\pm$ 0.06} & 41.97{\tiny $\pm$ 1.01} & 45.77{\tiny $\pm$ 0.28} & 44.28{\tiny $\pm$ 0.45} & 44.80{\tiny $\pm$ 0.63} & 65.15{\tiny $\pm$ 3.66} & 77.03{\tiny $\pm$ 0.25} & 79.91{\tiny $\pm$ 0.13} \\ 
      
      SphereFed~\cite{dong2022spherefed} & 42.71{\tiny $\pm$ 0.65} & 48.63{\tiny $\pm$ 0.90} & {\mybold{52.16}}{\tiny $\pm$ 0.22} & \mybold{53.41}{\tiny $\pm$ 0.19} & \mybold{76.33}{\tiny $\pm$ 0.33} & 83.67{\tiny $\pm$ 0.18} & 84.36{\tiny $\pm$ 0.30} & 39.56{\tiny $\pm$ 0.48} & 46.54{\tiny $\pm$ 0.58} & \mybold{49.41}{\tiny $\pm$ 0.78} & 49.22{\tiny $\pm$ 0.86} & 67.49{\tiny $\pm$ 3.49} & 80.05{\tiny $\pm$ 0.40} & {\mybold{82.62}}{\tiny $\pm$ 0.66} \\ 
      FedETF~\cite{li2023no} & 31.37{\tiny $\pm$ 0.72} & 42.22{\tiny $\pm$ 0.77} & 47.47{\tiny $\pm$ 0.67} & 49.00{\tiny $\pm$ 0.74} & 67.81{\tiny $\pm$ 0.94} & 80.78{\tiny $\pm$ 0.68} & 82.60{\tiny $\pm$ 0.46} & 40.71{\tiny $\pm$ 0.90} & 45.63{\tiny $\pm$ 0.33} & 46.28{\tiny $\pm$ 1.05} & 46.69{\tiny $\pm$ 0.87} & 70.75{\tiny $\pm$ 0.36} & 77.86{\tiny $\pm$ 0.46} & 79.95{\tiny $\pm$ 0.34} \\ 
      \alg \textbf{(Ours)} & \mybold{48.21}{\tiny $\pm$ 0.56} & \mybold{50.77}{\tiny $\pm$ 0.14} & {\mybold{52.15}}{\tiny $\pm$ 0.03} & \mybold{52.41}{\tiny $\pm$ 0.81} & \mybold{76.57}{\tiny $\pm$ 0.51} & 83.22{\tiny $\pm$ 0.34} & 84.14{\tiny $\pm$ 0.27} & \mybold{45.12}{\tiny $\pm$ 1.00} & \mybold{49.48}{\tiny $\pm$ 0.50} & \mybold{50.67}{\tiny $\pm$ 0.88} & \mybold{51.15}{\tiny $\pm$ 0.65} & \mybold{72.07}{\tiny $\pm$ 2.26} & \mybold{80.90}{\tiny $\pm$ 0.02} & {\mybold{82.42}}{\tiny $\pm$ 0.10} \\ \bottomrule
    \end{tabular}
    }
    % \vspace{-10pt}
\end{table*}

==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/tables/pfl.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{0.95}
\caption{PFL accuracy comparison over clients from a single seed.
$\mathrm{acc}^{t}$ is the accuracy after $t$ local fine-tuning steps, reported
as mean$_{\pm\text{std}}$; $\mathrm{acc}^{0}$ is given as the mean only.
Multi CL requires known groups and is not deployable on real annotators
(``--''). \textbf{Bold} marks the best value in each post-adaptation column.}
\label{tab:pfl}
\vspace{-8pt}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{Balanced (Synthetic)}
& \multicolumn{3}{c}{Imbalanced (Synthetic)}
& \multicolumn{3}{c}{Real-world} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
Algorithm & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{10}$ & $\mathrm{acc}^{80}$
          & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{10}$ & $\mathrm{acc}^{80}$
          & $\mathrm{acc}^{0}$ & $\mathrm{acc}^{80}$ & $\mathrm{acc}^{240}$ \\
\midrule
Local
  & 49.20 & $\acc{49.95}{7.26}$ & $\acc{58.05}{7.69}$
  & 50.25 & $\acc{51.30}{7.44}$ & $\acc{58.70}{7.07}$
  & 51.24 & $\acc{52.12}{6.65}$ & $\acc{54.59}{7.66}$ \\
\midrule
CL
  & 51.80 & $\acc{53.70}{7.15}$ & $\acc{55.40}{5.99}$
  & 56.00 & $\acc{56.90}{10.89}$ & $\acc{62.60}{7.93}$
  & 58.06 & $\acc{57.06}{9.08}$ & $\acc{61.00}{6.69}$ \\
Multi CL
  & 92.10 & $\acc{92.15}{3.88}$ & $\acc{91.60}{4.29}$
  & 92.30 & $\acc{91.70}{3.63}$ & $\acc{91.60}{3.67}$
  & -- & -- & -- \\
FL~\cite{mcmahan2017communication}
  & 50.35 & $\acc{92.45}{3.76}$ & $\mathbf{\acc{94.70}{2.92}}$
  & 55.60 & $\acc{90.55}{5.20}$ & $\mathbf{\acc{93.80}{3.40}}$
  & 60.82 & $\acc{61.53}{7.70}$ & $\acc{63.00}{9.10}$ \\
\midrule
FedBiscuit~\cite{wu2024towards}
  & 68.80 & $\acc{66.90}{6.18}$ & $\acc{71.45}{10.35}$
  & 78.45 & $\acc{77.85}{9.85}$ & $\acc{80.80}{8.46}$
  & 59.12 & $\acc{58.53}{6.76}$ & $\acc{57.06}{5.77}$ \\
Soft-FL
  & 51.70 & $\acc{62.40}{7.51}$ & $\acc{71.30}{6.09}$
  & 56.50 & $\acc{75.95}{9.81}$ & $\acc{86.20}{7.41}$
  & 60.88 & $\acc{58.71}{7.45}$ & $\acc{57.00}{9.07}$ \\
\alg (ours)
  & 49.15 & $\mathbf{\acc{94.55}{3.58}}$ & $\acc{94.30}{3.86}$
  & 54.95 & $\mathbf{\acc{92.35}{4.02}}$ & $\acc{93.75}{3.89}$
  & 60.59 & $\mathbf{\acc{61.71}{5.98}}$ & $\mathbf{\acc{64.41}{6.79}}$ \\
\bottomrule
\end{tabular}
}
\end{table*}


==> hhvskwqztgzzkcgnbpymvsykkwcyyctb/tables/pfl_acc.tex <==
\begin{table*}[h!]
    \centering
    \caption{PFL accuracy comparison with MobileNet on CIFAR-100. For PFL, we denote the entries in the form of X{\tiny $\pm$(Y)}, representing the mean and standard deviation of personalized accuracies across all clients derived from a single seed.}
    \label{tab:pfl_acc}
    \small
    \vspace{-10pt}
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{l|ccc|ccc}
    \toprule
    Algorithm & $s$=10 & $s$=20 & $s$=100 & $\alpha$=0.05 & $\alpha$=0.1 & $\alpha$=0.3 \\ \midrule
    Local only ($\mathcal{L}_\text{CE}$)                              & 58.05{\tiny $\pm$(8.11)}  & 42.45{\tiny $\pm$(6.44)} & 18.69{\tiny $\pm$(3.28)} & 55.39{\tiny $\pm$(8.79)}   & 43.76{\tiny $\pm$(7.46)} & 27.75{\tiny $\pm$(5.32)} \\
    
    Local only ($\mathcal{L}_\text{CE}$+ETF)
     & 58.01{\tiny $\pm$(7.34)}   & 41.62{\tiny $\pm$(5.91)} & 18.92{\tiny $\pm$(3.00)} & 55.34{\tiny $\pm$(9.13)}  & 43.37{\tiny $\pm$(7.12)} & 27.87{\tiny $\pm$(5.34)} \\ 
        
    % Local only (CE+ETF, Body)                               & 58.53{\tiny $\pm$(7.25)}   & 42.03{\tiny $\pm$(5.95)} & 19.25{\tiny $\pm$(3.46)} & 56.67{\tiny $\pm$(8.83)}  & 44.47{\tiny $\pm$(7.49)} & 28.52{\tiny $\pm$(5.34)} \\   

    Local only ($\mathcal{L}_\text{DR}$)                               & 60.68{\tiny $\pm$(7.77)}   & 44.61{\tiny $\pm$(6.61)} & 20.98{\tiny $\pm$(3.49)} & 58.56{\tiny $\pm$(9.16)}  & 46.72{\tiny $\pm$(7.29)} & 30.88{\tiny $\pm$(5.33)} \\    
    % Local only (DR)                               & 61.73{\tiny $\pm$(7.89)} & 44.35{\tiny $\pm$(5.98)}   & 21.13{\tiny $\pm$(3.71)} & 58.84{\tiny $\pm$(9.19)}  & 47.16{\tiny $\pm$(7.48)} &  31.35{\tiny $\pm$(5.41)} \\    
    
    \midrule
    FedPer~\cite{arivazhagan2019federated}                            & 70.67{\tiny $\pm$(7.19)}  & 57.27{\tiny $\pm$6.66} & 24.30{\tiny $\pm$(4.34)} & 62.67{\tiny $\pm$(7.65)}  & 53.43{\tiny $\pm$(6.60)} & 35.68{\tiny $\pm$(4.82)} \\ 
    Per-FedAvg~\cite{fallah2020personalized}                            & 32.13{\tiny $\pm$(10.90)}  & 36.66{\tiny $\pm$(8.86)} & 41.27{\tiny $\pm$(7.43)} & 28.81{\tiny $\pm$(8.68)}  & 35.56{\tiny $\pm$(6.56)} & 42.80{\tiny $\pm$(4.76)} \\ 
    
    FedRep~\cite{collins2021exploiting}                            & 63.14{\tiny $\pm$(7.63)}  & 51.69{\tiny $\pm$(6.50)} & 26.31{\tiny $\pm$(4.74)} &  57.53{\tiny $\pm$(8.05)}  & 49.60{\tiny $\pm$(6.25)} & 37.00{\tiny $\pm$(4.82)} \\ 
    
    Ditto~\cite{li2021ditto}                            & 39.26{\tiny $\pm$(14.43)}  & 38.18{\tiny $\pm$(9.96)} & 44.53{\tiny $\pm$(5.08)} & 35.81{\tiny $\pm$(14.83)}  & 37.81{\tiny $\pm$(11.80)} & 43.72{\tiny $\pm$(5.12)} \\ \midrule

    FedAvg-FT~\cite{mcmahan2017communication} & 69.81{\tiny $\pm$(6.78)}  & 56.13{\tiny $\pm$(5.77)} & 47.66{\tiny $\pm$(5.20)} & 63.37{\tiny $\pm$(9.28)}  & 56.79{\tiny $\pm$(5.96)} & 50.12{\tiny $\pm$(3.67)} \\ 

    FedBABU-FT~\cite{oh2021fedbabu} & 80.14{\tiny $\pm$(6.25)}  & 70.89{\tiny $\pm$(5.60)} & 52.14{\tiny $\pm$(5.09)} & 75.50{\tiny $\pm$(6.40)}  & 70.83{\tiny $\pm$(5.06)} & 56.91{\tiny $\pm$(3.74)} \\
    
    SphereFed-FT~\cite{dong2022spherefed} & 81.90{\tiny $\pm$(5.86)}  & 71.56{\tiny $\pm$(5.78)} & 55.83{\tiny $\pm$(4.67)} & 73.21{\tiny $\pm$(7.08)}  & 70.00{\tiny $\pm$(5.09)} & 60.03{\tiny $\pm$(3.99)} \\ 
    
    FedETF-FT~\cite{li2023no} & 53.75{\tiny $\pm$(7.35)}  & 52.94{\tiny $\pm$(5.71)} & 51.69{\tiny $\pm$(5.03)} & 52.96{\tiny $\pm$(8.01)}  & 53.97{\tiny $\pm$(5.40)} & 51.67{\tiny $\pm$(3.83)} \\ \midrule

    \textbf{{\alg}\,FT (ours)} & \textbf{84.10}{\tiny $\pm$(5.43)}  & \textbf{75.42}{\tiny $\pm$(4.80)} & \textbf{56.76}{\tiny $\pm$(4.91)} & \textbf{78.55}{\tiny $\pm$(6.16)}  & \textbf{74.75}{\tiny $\pm$(4.75)} & \textbf{62.16}{\tiny $\pm$(3.73)} \\ 
    \bottomrule
    \end{tabular}
    }
    % \vspace{-10pt}
\end{table*}

